Benchmarking Distributed Stream Data Processing Systems

The need for scalable and efficient stream analysis has led to the development of many open-source streaming data processing systems (SDPSs) with highly diverging capabilities and performance characteristics. While first initiatives try to compare the systems for simple workloads, there is a clear gap of detailed analyses of the systems' performance characteristics. In this paper, we propose a framework for benchmarking distributed stream processing engines. We use our suite to evaluate the performance of three widely used SDPSs in detail, namely Apache Storm, Apache Spark, and Apache Flink. Our evaluation focuses in particular on measuring the throughput and latency of windowed operations, which are the basic type of operations in stream analytics. For this benchmark, we design workloads based on real-life, industrial use-cases inspired by the online gaming industry. The contribution of our work is threefold. First, we give a definition of latency and throughput for stateful operators. Second, we carefully separate the system under test and driver, in order to correctly represent the open world model of typical stream processing deployments and can, therefore, measure system performance under realistic conditions. Third, we build the first benchmarking framework to define and test the sustainable performance of streaming systems. Our detailed evaluation highlights the individual characteristics and use-cases of each system.

==> 3_Preliminary.tex <==
%!TEX root = icde2018.tex
\section{PRELIMINARIES AND BACKGROUND}
\label{pre}

In this section, we provide background information about the stream data processing engines and their features used in this paper. 
We analyze Apache Storm, Apache Spark, and Apache Flink as they are the most mature and accepted ones in both academia and industry.


\subsection{Apache Storm}

Apache Storm is a distributed stream processing framework, which was open sourced after being acquired by Twitter \cite{storm}. 

Storm operates on tuple streams and provides record-by-record stream processing. 
It supports an at-least-once processing  semantics and guarantees all tuples to be processed. 
In cases of failure, events are replayed. 
Storm also supports exactly-once processing semantics with its Trident abstraction \cite{trident}. 

Stream processing programs are represented by a computational topology, which consists of spouts and bolts. 
Spouts are source operators and bolts are processing and sink operators. 
A Storm topology forms a directed acyclic graph (DAG), where the edges are tuple streams and vertices are operators (bolts and spouts). 
When a spout or bolt emits a tuple, the bolts that are subscribed to this spout or bolt receive input. 


Storm's lower level APIs provide only limited support for automatic memory and state management. 
Therefore, choosing the right data structure for state management and utilizing memory efficiently by making computations incrementally  is up to the user. 
Storm supports caching and batching the state transition. 
However, the efficiency of a particular operation degrades as the size of the state grows. 




Storm has built-in support for windowing. 
Although the information of expired, newly arrived, and total tuples within a window is provided through APIs, the incremental state management is not transparent to the users. 
Trident, on the other hand,  has built-in support for partitioned windowed joins and aggregations. 
Storm supports sliding and tumbling windows on processing time and event time. 
For event-time windows, tuples need to have a dedicated timestamp field so that the engine can create periodic watermarks. 
Any worker process in Storm topology sends acknowledgments to the source executor for a processed tuple. 
In case of failure Storm sends the messages again. 
A downside of acknowledgments in Storm is that tuples can be only be acknowledged once they are completely flushed out of a window by the operator. 
This is especially problematic for long windows with small slide.

Backpressure is one of the key features of SDPSs. 
It refers to the situation where a system is receiving data at a higher rate than it can process. 
For example, this can occur during temporary load spikes. 
Storm supports backpressure although the feature is not mature yet \cite{WinNT}. 
This was confirmed throughout our experiments as well. 


Storm uses an extra backpressure thread inside the system. 
Once the receiver queue of an operator is full, the backpressure thread is notified. 
This way Storm can notify all workers that the system is overloaded. 
Due to its high complexity, Storm's backpressure feature can stall the system and, therefore, it is not enabled by default in the current version.


\subsection{Apache Spark}
Apache Spark is an open source big data processing engine, originally developed at the University of California, Berkeley \cite{spark}. 
Unlike Storm and Flink, which support one record at a time, Spark Streaming inherits its architecture from batch processing, which supports processing records in micro-batches. 
Throughout this paper, we refer to Spark Streaming as simply Spark. 
The Resilient Distributed Dataset (RDD) is a fault-tolerant abstraction of Spark, which enables in-memory, parallel computation in  distributed cluster environments \cite{zaharia2012resilient}. 



One of Spark's features is its support of lazy evaluation. 
This enables the engine to run more efficiently. 
Spark  supports stage-oriented scheduling. 
Initially, it computes a DAG  of stages for each submitted job. 
Then it keeps track of materialized  RDDs and outputs from each  stage, and finally finds a minimal schedule. 
Unlike Flink and Storm, which also work based on DAG execution graphs, Spark's computing unit in a graph (edge) is a data set rather than streaming records and each vertex in a graph is a stage rather than individual operators. 
RDDs are guaranteed to be processed in order in a single DStream (Discretized Stream), which  is a continuous sequence of RDDs. 
However, there is no guaranteed ordering within RDDs  since each RDD is processed in parallel. 


Spark has improved its memory management significantly in the recent releases. 
The system shares the memory  between execution and storage. 
This unified memory management supports dynamic memory management between the two modules. 
Moreover, Spark supports dynamic memory management throughout the tasks and within operators of each task. 


Spark has a built-in support for windowed calculations. 
It supports only windows defined by processing time. 
The window size must be a multiple of the batch interval, because a window keeps a particular number of batches until it is purged. 
Choosing the  batch interval can heavily affect the performance of window-based analytics. 
First, the latency and response time of windowed analytics is strongly relying on the batch interval. 
Second, supporting only processing time windowed analytics, can be a severe limitation for some use-cases.


Spark also supports backpressure. 
It handles backpressure by putting a bound to the block size. 
Depending on the duration and load of each mini-batch job, the effectiveness of backpressure signal handling from source to destination may vary. 

%todo[inline]{fast enough for what?=>fixed}

\subsection{Apache Flink}
Apache Flink started off as an open source big data processing system at TU Berlin, leveraging in major parts the codebase of the Stratosphere project [9].
At its core, Flink is a distributed dataflow engine. 
Like in Storm, a Flink runtime program is a DAG of operators connected with data streams. 
Flink's runtime engine supports unified processing of batch (bounded) and stream (unbounded) data, considering former as being the special case of the latter.

Flink provides its own memory management to avoid long running JVM's garbage collector stalls by serializing data into memory segments. 
The data exchange in distributed environments is achieved via buffers. 
A producer takes a buffer from the pool, fills it up with data, then the consumer receives the data and frees the buffer informing the memory manager. 
Flink provides a wide range of high level and user friendly APIs to manage  state. 
Incremental state update, managing the memory, or checkpointing with big states are performed automatically and transparently to user. 


Flink has a strong feature set for building and evaluating windows on data streams. 
With a wide range of pre-defined windowing operators, it supports user-defined windows with custom logic. 
The engine provides processing-time, event-time, and ingestion-time semantics. 
When using processing time, like Spark, windows are defined with respect to the wall clock of the machine that is responsible for building and processing  a window. 
When using event time, on the other hand, the notion of time is determined by the timestamp attached to an event, which typically resembles its creation time. 
Like in Storm, the timestamps must be attached to each event record as a separate field. 
At ingestion time, the system processes records with event time semantics on these timestamps. 
Flink has support for out-of-order streams, which were motivated from Googles MillWheel and Dataflow papers \cite{akidau2013millwheel,akidau2015dataflow}. 
Flink also supports backpressure. 
It uses blocking queues. 
Once the congestion is detected this information is automatically transferred to upstream operators at negligible cost. 




==> Makefile <==
pdf:
	mkdir -p build
	@TEXINPUTS=.//: pdflatex -synctex=1 -interaction=nonstopmode -output-directory=build --shell-escape icde2018
all:
	mkdir -p build
	@TEXINPUTS=.//: pdflatex -synctex=1 -interaction=nonstopmode -output-directory=build --shell-escape icde2018
	bibtex build/icde2018
	pdflatex -synctex=1 -interaction=nonstopmode -output-directory=build icde2018
	pdflatex -synctex=1 -interaction=nonstopmode -output-directory=build icde2018
fig:
	rm figures/cache/*
	pdflatex -interaction=nonstopmode -output-directory build --shell-escape icde2018
clean:
	rm -rf build
	find . -type f \( -name  '*.thm' -or -name 'icde2018.pdf' -or -name '*.aux' -or -name  '*.auxlock' -or -name '*.figlist' -or -name '*eps-converted-to.pdf' -or -name '*.bbl' -or -name '*.fdb_latexmk' -or -name '*.synctex.gz' -or -name '*.blg' -or -name '*.log' -or -name '*.out' -or -name '*.toc' -or -name '*.lot' -or -name '*.lof' -or -name '*.loa' -or -name '*.fls' \) -exec rm -f '{}' \;
edit:
	subl paper.sublime-project


==> Stream Benchmarks ICDE18/0_Abstract.tex <==
%!TEX root = icde2018.tex
\begin{abstract}
	% With the increasing demand of online data processing and analysis, stream data processing has been gaining attention both in industry and in academia. 
	The need for scalable and efficient stream analysis has led to the development of many open-source streaming data processing systems (SDPSs) with highly diverging capabilities and performance characteristics. 
	While first initiatives try to compare the systems for simple workloads, there is a clear gap of detailed analyses of the systems' performance characteristics.
	In this paper, we propose a framework for benchmarking distributed stream processing engines. 
	We use our suite to evaluate the performance of three widely used SDPSs in detail, namely Apache Storm, Apache Spark, and Apache Flink. 
	Our evaluation focuses in particular on measuring the throughput and latency of windowed operations, which are the basic type of operations in stream analytics. 
	For this benchmark, we design workloads based on real-life, industrial use-cases inspired by the online gaming industry. 
	The contribution of our work is threefold.
	First, we give a definition of latency and throughput for stateful operators. 
	Second, we carefully separate the system under test and driver, in order to correctly represent the open world model of typical stream processing deployments and can, therefore, measure system performance under realistic conditions.
	Third, we build the first benchmarking framework to define and test the sustainable performance of  streaming systems.
	Our detailed evaluation highlights the individual characteristics and use-cases of each system.
\end{abstract}


==> Stream Benchmarks ICDE18/1_Introduction.tex <==
%!TEX root = icde2018.tex

\section{Introduction}
Processing large volumes of data in batch is often not sufficient in cases where new data has to be processed fast to quickly adapt and react to changes. 
For that reason, stream data processing  has gained significant attention. 
The most popular streaming engines, with large-scale adoption in industry and the research community, are Apache Storm \cite{toshniwal2014storm}, Apache Spark  \cite{zaharia2012discretized}, and Apache Flink \cite{carbone2015apache}. 
As a measure for popularity, we consider the engines' community size, pull requests, number of contributors, commit frequency at the source repositories, and the size of the industrial community adopting the respective systems in their production environment.


An  important application area of stream data processing is  online video games. 
These require the fast processing  of large scale online data feeds  from different sources. 
Windowed aggregations and windowed joins are two main operations that are used to monitor user feeds. 
A typical use-case is tracking the in-application-purchases per application, distribution channel, or product item (in-app products). 
Another typical use-case is the monitoring of advertising:  making sure that all campaigns and advertisement networks work flawlessly, and comparing different user feeds by  joining them. 
For example, monitoring the in-application-purchases of the same game downloaded from different distribution channels and comparing users'  actions  are essential in  online video game monitoring.


In this work, we propose a benchmarking framework to accurately measure the performance of SDPSs. 
For our experimental evaluation, we test three publicly available open source engines: Apache Storm, Apache Spark, and Apache Flink. 
%
We use latency and throughput as the two major performance indicators. 
Latency, in SDPS, is the time difference between the moment of data production at the source (e.g., the mobile device) and the  moment that the tuple has produced an output. 
Throughput, in this scenario, determines the number of ingested and processed records per time unit.


Even though there have been several comparisons of the performance of SDPS recently, they did not measure the latency and throughput that can be achieved in a production setting. 
One of the repeating issues in previous works is the missing definition and inaccurate measurement of latency in stateful operators (e.g., joins). 
Moreover, previous works do not clearly separate the system under test (SUT) and the benchmark driver. 
Frequently, the performance metrics are measured and calculated within the SUT resulting in incorrect measurements.
% We discuss in detail these challenges as well as our solutions in Section \ref{chal}.


In this paper, we address the above mentioned challenges. 
Our proposed benchmarking framework is generic with a clear design and well defined metrics, which can be applied to a number of different stream execution engines. 
% Our main goal is to stimulate an environment in which we can measure the metrics more precisely and with minimum influence of side factors. 
The main contributions of this paper are as follows:
\begin{itemize}
	\item We introduce a mechanism to accurately measure the latency of stateful operators in SDPSs. 
	We apply the proposed method to various use-cases. 
	\item We accomplish the complete separation of the test driver from the system under test. 
	\item We measure the maximum sustainable throughput of a SDPSs. 
	Our benchmarking framework handles system specific features like backpressure to measure the maximum sustainable throughput of a system. 
	\item We use the proposed benchmarking system for an extensive evaluation of Storm, Spark, and Flink with practical use-cases.
\end{itemize}




==> Stream Benchmarks ICDE18/2_Related_Work.tex <==
%!TEX root = icde2018.tex
\section{Related work}
\label{rel}

Benchmarking parallel data processing systems has been an active area of research. Early benchmarking efforts have focused on batch processing and later on extended to stream processing.

\para{Batch Processing.}
HiBench~\cite{huang2011hibench} was the first benchmark suite to evaluate and characterize the performance of Hadoop and it was later extended with a streaming component~\cite{white2012hadoop}.
HiBench includes a wide range of experiments ranging from micro-benchmarks to machine learning algorithms. 
SparkBench, features machine learning, graph computation, SQL queries, and streaming applications on top of Apache Spark~\cite{li2015sparkbench}.
BigBench~\cite{ghazal2013bigbench} built an end-to-end benchmark with all major characteristics in the lifecycle of big data systems.
The BigDataBench~\cite{wang2014bigdatabench} suite contains  19 scenarios covering a broad range of applications and diverse data sets. Marcu et al.~\cite{marcu2016spark}
performed  an extensive analysis of the differences between Apache Spark and Apache Flink on iterative workloads. The above benchmarks either adopt batch processing systems and metrics used in batch processing systems or apply the batch-based metrics on SDPSs. We, on the other hand, analyze streaming systems with a new definition of metrics and show that adopting batch   processing metrics for SDPSs leads to biased benchmark results. 


\para{Stream Processing.} 
Recently, a team from Yahoo! conducted an informal series of experiments on three Apache projects, namely Storm, Flink, and Spark and measured their latency and throughput \cite{chintapalli2016benchmarking}. 
They used Apache Kafka \cite{kreps2011kafka} and Redis \cite{carlson2013redis} for data retrieval and storage respectively. 
Perera et al. used the Yahoo Streaming Benchmark and Karamel \cite{karamel} to provide reproducible batch and streaming benchmarks of Apache Spark and Apache Flink in a cloud environment \cite{perera2016reproducible}. 
Later on, it was shown \cite{dataartisans} that Kafka and Redis were the bottleneck in the experiments of the Yahoo! Streaming Benchmark \cite{chintapalli2016benchmarking} and transitively to \cite{perera2016reproducible}. 
%However, for other metrics such as CPU usage and latency, we notice significant differences. 
%The authors used the Yahoo! Stream Benchmark (YSB) for their evaluation. 
%As mentioned above, YSB has several bottlenecks, which explains the differences. 
In this paper, we overcome those  bottlenecks by $i)$~generating the data on the fly with a scalable data generator (Section \ref{des}) instead of ingesting data from Kafka and $ii)$~not storing data in a key-value store. 


Lopez et al.~\cite{lopez2016performance} propose a benchmarking framework to assess the throughput performance of Apache Storm, Spark, and Flink under node failures. 
The key finding of their work is that Spark is more robust to node failures but it performs up to an order of magnitude worse than Storm and Flink. 
Compared to this work, we observed a large difference with respect to the throughput achieved by the same systems. 
The paper in question allows the systems to ingest data at maximum rate. 
Instead, we introduce the concept of sustainable throughput: in our experiments we control the data ingestion rate (throughput) of a system, in order to avoid large latency fluctuations. 
We argue that  sustainable throughput is a more representative metric which takes into account the latency of a system.

Shukla et al.~\cite{shukla2016benchmarking} perform common IoT tasks with different SDPSs, evaluating their performance. 
The authors define latency as the interval between the source operator's \emph{ingestion} time and the sink operator's result \emph{emission} time. 
As we discuss in Section~\ref{sec_metrics}, this approach leads to inaccurate measurements as the effects of backpressure and other effects are not visible in the results. The same issue is also present in the LinearRoad benchmark~\cite{arasu2004linear}. To alleviate this problem, we perform experiments measuring \emph{event-time latency}. 
Additionally, Shukla et al. define throughput  as the  rate of \emph{output} messages emitted from the output operators in a unit time. 
However, since the number of result-tuples can differ from the input-tuples (e.g., in an aggregation query) we measure the throughput of \emph{data ingestion} and introduce the concept of sustainable throughput.

StreamBench~\cite{lu2014stream}, proposes a method to measure the throughput and latency of a SDPS with the use of a mediator system between the data source and the SUT. 
In this work, we explain that such a mediator system is  a bottleneck and/or affect the measurements' accuracy. 
Finally, several stream processing systems implement their own benchmarks to measure the system performance without comparing them with any other system~\cite{neumeyer2010s4,qian2013timestream,zaharia2012discretized}. 

In summary, our benchmark framework is the first to $i)$~separate the SUT and driver, $ii)$~use a scalable data generator and to $iii)$~define metrics for system-, and event-time, as well as to $iv)$~introduce and use the concept of sustainable throughput throughout experiments.




==> Stream Benchmarks ICDE18/3_Preliminary.tex <==
%!TEX root = icde2018.tex
\section{PRELIMINARIES AND BACKGROUND}
\label{pre}

In this section, we provide background information about the stream data processing engines and their features used in this paper. 
We analyze Apache Storm, Apache Spark, and Apache Flink as they are the most mature and accepted ones in both academia and industry.


\subsection{Apache Storm}

Apache Storm is a distributed stream processing framework, which was open sourced after being acquired by Twitter \cite{storm}. 

Storm operates on tuple streams and provides record-by-record stream processing. 
It supports an at-least-once processing  semantics and guarantees all tuples to be processed. 
In cases of failure, events are replayed. 
Storm also supports exactly-once processing semantics with its Trident abstraction \cite{trident}. 

Stream processing programs are represented by a computational topology, which consists of spouts and bolts. 
Spouts are source operators and bolts are processing and sink operators. 
A Storm topology forms a directed acyclic graph (DAG), where the edges are tuple streams and vertices are operators (bolts and spouts). 
When a spout or bolt emits a tuple, the bolts that are subscribed to this spout or bolt receive input. 


Storm's lower level APIs provide only limited support for automatic memory and state management. 
Therefore, choosing the right data structure for state management and utilizing memory efficiently by making computations incrementally  is up to the user. 
Storm supports caching and batching the state transition. 
However, the efficiency of a particular operation degrades as the size of the state grows. 




Storm has built-in support for windowing. 
Although the information of expired, newly arrived, and total tuples within a window is provided through APIs, the incremental state management is not transparent to the users. 
Trident, on the other hand,  has built-in support for partitioned windowed joins and aggregations. 
Storm supports sliding and tumbling windows on processing time and event time. 
For event-time windows, tuples need to have a dedicated timestamp field so that the engine can create periodic watermarks. 
Any worker process in Storm topology sends acknowledgments to the source executor for a processed tuple. 
In case of failure Storm sends the messages again. 
A downside of acknowledgments in Storm is that tuples can be only be acknowledged once they are completely flushed out of a window by the operator. 
This is especially problematic for long windows with small slide.

Backpressure is one of the key features of SDPSs. 
It refers to the situation where a system is receiving data at a higher rate than it can process. 
For example, this can occur during temporary load spikes. 
Storm supports backpressure although the feature is not mature yet \cite{WinNT}. 
This was confirmed throughout our experiments as well. 


Storm uses an extra backpressure thread inside the system. 
Once the receiver queue of an operator is full, the backpressure thread is notified. 
This way Storm can notify all workers that the system is overloaded. 
Due to its high complexity, Storm's backpressure feature can stall the system and, therefore, it is not enabled by default in the current version.


\subsection{Apache Spark}
Apache Spark is an open source big data processing engine, originally developed at the University of California, Berkeley \cite{spark}. 
Unlike Storm and Flink, which support one record at a time, Spark Streaming inherits its architecture from batch processing, which supports processing records in micro-batches. 
Throughout this paper, we refer to Spark Streaming as simply Spark. 
The Resilient Distributed Dataset (RDD) is a fault-tolerant abstraction of Spark, which enables in-memory, parallel computation in  distributed cluster environments \cite{zaharia2012resilient}. 



One of Spark's features is its support of lazy evaluation. 
This enables the engine to run more efficiently. 
Spark  supports stage-oriented scheduling. 
Initially, it computes a DAG  of stages for each submitted job. 
Then it keeps track of materialized  RDDs and outputs from each  stage, and finally finds a minimal schedule. 
Unlike Flink and Storm, which also work based on DAG execution graphs, Spark's computing unit in a graph (edge) is a data set rather than streaming records and each vertex in a graph is a stage rather than individual operators. 
RDDs are guaranteed to be processed in order in a single DStream (Discretized Stream), which  is a continuous sequence of RDDs. 
However, there is no guaranteed ordering within RDDs  since each RDD is processed in parallel. 


Spark has improved its memory management significantly in the recent releases. 
The system shares the memory  between execution and storage. 
This unified memory management supports dynamic memory management between the two modules. 
Moreover, Spark supports dynamic memory management throughout the tasks and within operators of each task. 


Spark has a built-in support for windowed calculations. 
It supports only windows defined by processing time. 
The window size must be a multiple of the batch interval, because a window keeps a particular number of batches until it is purged. 
Choosing the  batch interval can heavily affect the performance of window-based analytics. 
First, the latency and response time of windowed analytics is strongly relying on the batch interval. 
Second, supporting only processing time windowed analytics, can be a severe limitation for some use-cases.


Spark also supports backpressure. 
It handles backpressure by putting a bound to the block size. 
Depending on the duration and load of each mini-batch job, the effectiveness of backpressure signal handling from source to destination may vary. 

%todo[inline]{fast enough for what?=>fixed}

\subsection{Apache Flink}
Apache Flink started off as an open source big data processing system at TU Berlin, leveraging in major parts the codebase of the Stratosphere project [9].
At its core, Flink is a distributed dataflow engine. 
Like in Storm, a Flink runtime program is a DAG of operators connected with data streams. 
Flink's runtime engine supports unified processing of batch (bounded) and stream (unbounded) data, considering former as being the special case of the latter.

Flink provides its own memory management to avoid long running JVM's garbage collector stalls by serializing data into memory segments. 
The data exchange in distributed environments is achieved via buffers. 
A producer takes a buffer from the pool, fills it up with data, then the consumer receives the data and frees the buffer informing the memory manager. 
Flink provides a wide range of high level and user friendly APIs to manage  state. 
Incremental state update, managing the memory, or checkpointing with big states are performed automatically and transparently to user. 


Flink has a strong feature set for building and evaluating windows on data streams. 
With a wide range of pre-defined windowing operators, it supports user-defined windows with custom logic. 
The engine provides processing-time, event-time, and ingestion-time semantics. 
When using processing time, like Spark, windows are defined with respect to the wall clock of the machine that is responsible for building and processing  a window. 
When using event time, on the other hand, the notion of time is determined by the timestamp attached to an event, which typically resembles its creation time. 
Like in Storm, the timestamps must be attached to each event record as a separate field. 
At ingestion time, the system processes records with event time semantics on these timestamps. 
Flink has support for out-of-order streams, which were motivated from Googles MillWheel and Dataflow papers \cite{akidau2013millwheel,akidau2015dataflow}. 
Flink also supports backpressure. 
It uses blocking queues. 
Once the congestion is detected this information is automatically transferred to upstream operators at negligible cost. 




==> Stream Benchmarks ICDE18/4_Challenges.tex <==
%!TEX root = icde2018.tex
% \section{Challenges \& Design Decisions}
% \label{chal}
% There are several challenges to be addressed when designing a benchmarking framework for SDPSs. 
% In this section, we analyze these challenges and explain our solutions.

% \begin{figure}
% 	%\captionsetup[subfigure]{aboveskip=3pt,belowskip=-4pt}
% 	\centering
% 	\begin{subfigure}[b]{0.16\textwidth}
% 		\includegraphics[width=\textwidth]{eps/no_queue}
% 		\caption{Without  queue}
% 		\label{fig_no_queue}
% 	\end{subfigure}\hspace{-1mm}%
% 	\begin{subfigure}[b]{0.16\textwidth}
% 		\includegraphics[width=\textwidth]{eps/yes_queue}
% 		\caption{With  queue}
% 		\label{fig_yes_queue}
% 	\end{subfigure}\hspace{-1mm}%
% 	\begin{subfigure}[b]{0.16\textwidth}
% 		\includegraphics[width=\textwidth]{eps/node_queue}
% 		\caption{Partial  queue}
% 		\label{fig_partial_queue}
% 	\end{subfigure}
% 	\caption{System designs to connect data generator and SUT.}
% 	\vspace{-2em}
% 	\label{fig_queue_link}
% \end{figure}




% \subsection{Metrics} The first metric we evaluate is throughput. We define throughput as the number of events that can be ingested in a given amount of time. 

% \para{Sustainable Throughput}
% If the system can ingest and process all the data produced by the driver instances during the whole experiment, then the system can \textit{sustain} the given throughput, we call this \textit{sustainable throughput}. 

% \para{Maximum Sustainable Throughput}
% If the system sustains the given throughput and cannot process more, we call it \textit{maximum sustainable throughput} (MST).

% In this paper, we analyze the MST of SDPSs which is  sum of the throughput of all driver instances. 
% So, we keep throughput assessment inside the driver instances and sum them at the end of experiment. 


% \para{Event-time Latency} Similar to the nomenclature of streaming systems \cite{carbone2015apache,akidau2013millwheel}, we define the \textit{event time latency} to be the interval between tuple's event time and emission time from SUT's sink operator. 


% \para{System-time Latency} The interval between a tuple's ingestion time to SUT and its emission time from the SUT's sink operator as \textit{system time latency}.
% We develop a model to calculate the latency of a stateful operator, which we analyze in Section \ref{sec_latency}.  

% ASterios: I removed this below as the discussionis quite shaky and can be easily attacked. There is not proof for what we claim...
% Our definition of latency can also be applied to push based data ingestion. 
% Because our industry setup adopts pull based data ingestion, in particular using Apache Kafka \cite{kreps2011kafka}, we conduct our experiments with pull based data ingestion. 
% Moreover, when pushing the data to an SDPS or generating input data inside the system, we need to allocate at least one operator of the system to do so. 
% Then, depending on a system architecture, we lose control over the precision of the metrics. 
% For example, when backpressure is active, this will affect the speed of data generator operator of a SDPS, because the operator is inside the SDPS. 
% Moreover, depending on several parameters such as system, query type, and parallelism  there is no guarantee that a system allocates a separate thread for the data generator operator. 
% For example, for some use-cases it is often beneficial  to set the parallelism of  SDPS slightly more than CPU count. 
% As a result, the system assigns different operator instances to the same computation slot (single thread in this case), which might affect the speed of data generation. 
% Considering these, we can conclude that push based data ingestion or data generation inside the SUT is theoretically the same as with pull  based data ingestion; however, system-specific issues need to be taken into consideration.



% to  tuples by selecting their maximum timestamp and appending the resulting timestamp to the emitted tuple from stateful operator. 
% In this way, we measure the latency of stateful computation time, excluding the tuples' 

% Benchmarks for far either concentrated on stateless operators or evaluated the latency of stateful operators by checkpointing to external systems. 
% As we discussed above, this approach can be a bottleneck and will influence the measurements. 







==> Stream Benchmarks ICDE18/5_System_Design.tex <==
%!TEX root = icde2018.tex
\section{Benchmark Design Decisions}
\label{des}
In this section, we  discuss the main design decisions of our benchmarking framework. We choose to generate data on-the-fly, rather than reading the data from a message broker or the filesystem and we use queues between the data generators and the streaming systems.








% Many systems continuously collect metrics inside the SUT while an application is running. 
% Using these measurements for benchmarking is problematic for several reasons. 
% First, if we utilize metric measurements directly from the SUT, benchmarking different systems is problematic especially if the semantics of metric measurements are different among systems or even the semantics is unknown if the system is blackbox. 
% Second, measuring latency and throughput inside the system or with clear separation from system gives completely different results,

\subsection{On-the-fly Data Generation vs. Message Brokers}
% The  between the data generator and the SUT can cause large additional overheads when benchmarking. 
% To test the SDPS, a data generator component is essential, to provide large amounts of streaming data. 
% Figure \ref{fig_queue_link} shows  three possible cases to link the data generator and the SUT. 
% The simplest design is to connect the SDPS directly to the data generators as shown in Figure \ref{fig_no_queue}. 
% Although this is a perfectly acceptable design, it does not match real-life use-cases. 
Streaming systems nowadays typically pull the data from message brokers, such as Apache Kafka~\cite{kreps2011kafka}, instead of directly connecting to push-based data sources. 
The message broker persists data coming from various sources~\cite{ranjan2014streaming}, allowing for data replication and making it available for other systems to use. 
The data exchange between the message broker and the streaming system may easily become the bottleneck of a benchmark deployment for a number of reasons. 
First, if the message broker's data partitioning is not chosen wisely, data re-partitioning may occur before the data reaches the sources of the streaming system.
This can happen when data resides in a different machine in the cluster or the data is partitioned in a different way than the streaming system requires it. 
Finally, the data needs to persist on disk before going through a de-/serialization layer between the streaming system and the message broker.
In our benchmark design, we choose to not use  a message broker, but rather, use a distributed in-memory data generator with configurable data generation rate. Before each experiment we benchmarked and distributed our data generator such that the data generation rate is faster than the data ingestion rate of the fastest system. 
This way, the communication between the data generator and the SUT is bounded only by the network bandwidth and the speed of the data ingestion by the SUT.

\subsection{Queues Between Data Generators and SUT Sources}
It is quite common that the data ingestion rate or throughput of a streaming system is not constant throughout the duration of an experiment. The fluctuations in the ingestion rate can be due to transient network issues, garbage collection in JVM-based engines, etc.
To alleviate this problem, we add a queue between each data generator and the SUT's source operators in order to even out the difference in the rates of data generation and data ingestion. 


\subsection{Separation of Driver and the SUT}
We choose to isolate the benchmark driver, i.e., the data generator, queues, and measurements from the SUT. 
In previous works, the throughput was either measured inside the SUT or the benchmark used internal statistics of the SUT.
However, different systems can have very diverse definitions  of latency and throughput leading.
In our benchmarking framework, we choose to separate the driver and the SUT, to perform measurements out of the SUT. 
More specifically, we measure throughput at the queues between the data generator and the SUT and measure latency at the sink operator of the SUT. 
Each pair of data generator and queue resides on the same machine to avoid any network overhead and to ensure data locality, while the queue data is always kept in memory to avoid disk write/read overhead. 


The data generator timestamps each event at generation time. It performs so, with constant speed throughout the experiment. 
The event's latency is calculated from the time instance that it is generated, i.e., the longer an event stays in a queue, the higher its  latency. 
We make sure that no driver instance runs on the same machines as the SUT  to affect its performance. 




\begin{figure*}[!htb]
	\centering
	\includegraphics[width=0.9\textwidth]{eps/usecase}
		
	\caption{End-to-end example of an aggregation query. The data generator produces tuples on a given event-time (before \texttt{time=600}), a second later the events enter the streaming system where they are grouped by their key, and finally aggregated (SUM). The event-time latency of the output tuple equals to the maximum event-time latency of elements in each window.}
	\label{agg_usecase}
\end{figure*}


\begin{figure*}[!htb]
	\centering
	\includegraphics[width=0.9\textwidth]{eps/joinwindows}
		
	\caption{End-to-end join of two streams. The generator creates events, which are then read by the streaming system and form a 10-minute window. The events are joined and the event-time of the result-tuples equals to the maximum event-time  of tuples in their corresponding windows.}
	\label{join_usecase}
\end{figure*}












\section{Metrics}
\label{sec_metrics}

Streaming systems are typically evaluated using two main metrics: throughput and latency. In this section, we make a distinction between two types of latency, namely event-time latency and processing-time latency. We then describe two types of throughput, namely maximum throughput and sustainable throughput. 

\subsection{Latency}

Modern streaming systems~\cite{akidau2015dataflow,carbone2015apache,akidau2013millwheel}  distinguish two notions of time: \textit{event-time} and \textit{processing-time}. 
The \textit{event-time} is the time when an event is captured while \textit{processing-time} is the time when an operator processes a tuple. Similar to the nomenclature of these two notions of time, we distinguish between event- and processing-time latency.

% \noindent\textit{Event-time latency.} 
\begin{definition}[Event-time Latency]
We define \emph{event-time latency} to be the interval between a tuple's event-time and its emission time from the SUT output operator. 
\end{definition}

For instance in an ATM transaction, the event-time is the moment of a user's action at the terminal, and the event-time latency is the time interval between the moment that the user's action took place and the moment that the event has been fully processed by the streaming system. 

\begin{definition}[Processing-time Latency]
We define \emph{processing-time latency} to be the interval between a tuple's \emph{ingestion} time (i.e., the time that the event has reached the input operator of the streaming system) and its emission time from the SUT output operator.  
\end{definition}
% \noindent\textit{System-time latency.} 




\para{Event- vs. processing-time latency.} Event- and processing-time latencies are equally important metrics. The event-time latency includes the time that a given event has spent in a queue, waiting to be processed, while processing-time latency is used to measure the time it took for the event to be processed by the streaming system. In practical scenarios, event-time latency is very important as it defines the time in which the user interacts with a given system and should be minimized. Clearly, processing-time latency makes part of the event-time latency. We use both metrics to characterize a system's performance.
Not clearly differentiating the two metrics leads to the coordinated omission problem. In coordinated omission service time (i.e., processing time) is measured at the SUT and any increasing queuing time, which is part of the \textit{response time} (i.e., event time), is ignored \cite{omission}. 
Friedrich et al. show that coordinated omission leads to significant underestimation of latencies \cite{friedrich2017coordinated}.





% One solution is  to measure the latency in the SDPS the same way as it is measured in batch data processing systems. 
% In this case, the number and complexity of the systems between SDPS and data source is irrelevant as the latency is the interval between tuples' ingestion and output from SUT. 
% However, this measurement of latency is too \textit{optimistic} and does not result in the real latency of the tuple. 
% The reason is that  the actual latency is based on tuples' event generation time. 

% Therefore, the usual method of measuring the latency within SDPS does not conform to real world scenarios especially in pull-based SDPSs. 
% Depending on their backpressure mechanism, a pull-based SDPS will reduce the input rate on high loads, which will not be reflected in the measured latency. 
% To solve this, we define the latency for SDPSs to be the difference between tuple's event time and output time. 



%The above challenge is called coordinated omission problem. 
%Basically, coordinated omission makes a user think that she is measuring \textit{response time} (i.e., event-time) when actually she measures only  \textit{service time} (system-time) \cite{omission}. 
%Friedrich et al. 
%show that ignoring this aspect can lead to significantly unrealistic results \cite{friedrich2017coordinated}.	

% Another factor triggering the unrealistic latency is the data generation rate. 
% If the input data rate is higher than the SDPS's MST and we measure the event time latency, the results may not exhibit the real latency. 
% Initially the system will try to ingest as much data as possible. 
% As a result, the SUT's processing time will take longer and the latency will increase for every adjacent tuple. 
% To solve this issue, we conduct experiments with our new definition of throughput (Section \ref{sec_metrics}) for  SDPSs. 



\para{Event-time Latency in Windowed Operators.} 
Stateful operators such as window aggregates (a sum aggregate over an hour's worth of data), retain state and return results after having seen a number of tuples over some time.
Measuring latency in such cases is non-trivial. 
The reason is that the latency of a given windowed operator is affected by the tuples' waiting time until the window is formed completely.


Figure \ref{agg_usecase} depicts the data generator, and a set of events in three queues. The events are timestamped with their event-time when they are generated. The events are then grouped by their key and are put in a 10-minute window.

Take, for example, the window containing the red events with \texttt{key=US}. The timestamps of these three events are of 580, 590, and 600. When these events are aggregated into a new event (the sum of their values with a total of \texttt{value=42}) we need to assign an event-time to that output. That event-time is then used to calculate the event-time latency on the operator output (in this case, \texttt{latency=10}). The main intuition is that in this way, we exclude the tuples' waiting time while the window is still buffering data. The event-time is defined more formally below.

\begin{definition}[Event-time of Windowed Events]
The event-time of a windowed operator's output event,  is the \emph{maximum event-time of all events that contributed to that output}.  
\end{definition}

In a windowed join operation, the containing tuples' event-time is set of be the maximum event-time of their window. Afterwards, each join output is assigned the maximum event-time of its matching tuples. As described in our example, in order to calculate the event-time latency of an output tuple, all we have to do is subtract the event-time of that tuple from the current system time. Figure \ref{join_usecase} shows the main intuition behind this idea. We join ads (yellow) and purchases (green) streams in a 10-minute window. 




\para{Processing-time Latency in Windowed Operators.} 
Apart from event-time latency, we need to calculate the processing-time latency of tuples as well. We define the processing-time of a windowed event similarly to the event-time.

\begin{definition}[Processing-time of Windowed Events]
The processing-time of a windowed operator's output event, is the \emph{maximum processing-time of all events that contributed to that output}.  
\end{definition}

The processing-time latency is calculated in exactly the same way as for event-time, with a small difference. Every tuple is enriched with an extra, processing-time field at its ingestion time (when it reached the first operator of the streaming system). In our example in Figure \ref{agg_usecase}, this happens right after \texttt{time=601}. To calculate the processing-time latency, we simply subtract the processing-time of that tuple from the current system time. 



% While the use-case provides the semantics for aggregating or joining tuples, the semantics for measuring the latency of stateful operators is unclear. 
% We provide efficient solution for this problem in our benchmarking framework.
% When the tuples arrive to a stateful operator, it does the aggregation that is defined in the use-case. 
% Besides the aggregation  defined in the use-case,  we aggregate the timestamp fields of tuples within stateful operator.

\subsection{Throughput}
The throughput of a data processing system is defined as the number of events that the system can process in a given amount of time. Throughput and event-time latency often do not correlate. For instance, a streaming system that batches tuples together before processing them, can generally achieve higher throughput. However, the time spent batching events affects the events' event-time latency. 

In practice, the deployment of a streaming system has to take into account the arrival rate of data. When the data arrival rate increases, the system has to adapt (e.g., by scaling out) in order to  handle the increased arrival rate and process tuples without exhibiting backpressure. To reflect this, we define the concept of \emph{sustainable throughput} and discuss how we attain it in our experiments.






\begin{figure}[!htb]
	\centering
	\includegraphics[width=0.5\textwidth]{eps/sustainability_axis}
		
	\caption{Sustainable throughput and unsustainable throughput}
	\label{fig:sustainable-throughput}
\end{figure}




\para{Sustainable Throughput.} When given more data than it can handle, a system starts to build up backpressure, i.e., the system queues up new events in order to process the events that have already been ingested. As a result, from the moment that backpressure mechanism is started, the event-time latency of all queued events increases. As we can see from Figure \ref{fig:sustainable-throughput},  backpressure can be transient: as soon as the system catches up again with the events' arrival rate, the event-time latency will stabilize. When the system's throughput is larger than the events' arrival rate, the event-time latency will decrease to the minimum (i.e., the processing-time).


\begin{definition}[Sustainable Throughput]
Sustainable throughput is the highest load of event traffic that a system can handle without exhibiting prolonged backpressure, i.e., without a continuously increasing event-time latency.
\end{definition}

In our experiments, we make sure that the data generation rate matches the sustainable throughput of a given deployment. To find the sustainable throughput of a given deployment we run each of the systems with a very high generation rate and we decrease it until the system can sustain that data generation rate. We allow for some fluctuation, i.e., we allow a maximum number of events to be queued, as soon as the queue does not continuously increase. 
% We provide more details on the allowed fluctuation in Section~\ref{eval}.



% \noindent{\color{red}FIXME: Asterios stopped here. Will continue tomorrow with defining criteria for spotting sustainable latency in practice.}
% Finding the sustainable throughput of a system is a non-trivial task. The goal is to match the data generation rate to the data ingestion rate of the system while allowing some small fluctuations, but no monotonically increasing event-time latency.

% \para{Maximum vs. sustainable througput.} 
% One may argue that the maximum thoughput a system can handle coincides with the sustainable thoughput. However, 




% In real-world applications, delays longer than a predefined threshold are unacceptable. 
% If the server is overloaded because of peaks, skews and etc., the player observes a loading screen. Depending on company regulations the acceptable length of delay thresholds can be different.

% If the system can ingest and process all the data produced by the driver instances during the whole experiment, then the system can \para{sustain} the given throughput.


% To examine if a system can sustain a given throughput, we divide the queue used in the DQI into two parts: $q^{a}$ and  $q^{b}$ (Figure \ref{fig_queue}). 
% If the size of the queue is less than or equal to $q^{a}$ throughout the experiment, then this is acceptable, meaning the SUT can sustain the given throughput. 
% If the queue size is between $q^{a}$ and  $q^{b}$ on the other hand, the SUT cannot sustain the given data rate, but the driver might tolerate it for some time. 
% A longer queue can be caused by slow system initialization, backpressure, etc. 
% However, if the queue size is longer than $q^{b}$ then the SUT cannot sustain the given throughput and the latency is expected to continuously increase. 
% In this case we end the experiment. 

% Our system supports user-defined policies to test the sustainability. 
% For example, one policy tolerates the $q^{b}$ part of the queue for a given time period (time based policy). 
% Another policy tolerates   the $q^{b}$ part of the queue for a given number of pushes into the queue (count based policy).
% This policy is customizable and can be easily plugged into the driver. 

% We choose a policy that is a combination of time and count based policies. 
% Once the queue size exceeds the $q^{a}$ and is less than $q^{b}$, we wait until $\frac{q^{b} - q^{a}}{2}  $ elements are pushed into the queue and check again. 
% If the queue size is still bigger than $q^{a}$, we end the benchmark concluding the SUT cannot sustain the given throughput. 
% We perform this process continuously in all DIs 
% If the SUT fails to sustain one instance of the driver, then the driver halts experiments  meaning the SUT cannot sustain the given throughput. 
% That is, the SUT can sustain a given workload if it can sustain the throughput of all DIs.

% It is crucial that the separation of the driver and the SUT and handling backpressure on the driver side does not cause side effects in metric measurements. 
% The driver does not stop the benchmark when the system exhibits backpressure. 
% An accurate selection of $q^{a}$ and $q^{b}$  is important. 
% In our experiments, first we assign  15\% and 30\% of input size for variables $q^{a}$, $q^{b}$ respectively. 
% In this case, the system can handle the given input; however, with longer experiments it fails, as the size of the queue keeps increasing. 
% Moreover, we get very large latencies for the given input. 
% As a result, we keep decreasing the variables until we find the best thresholds for all systems. 
% It is also important to clarify  that the value of  $q^{a}$  does not result   in biased experimental results because of its size (5\%). 
% We would like to draw reader's attention to the performance figures at Section \ref{eval}. 
% If the system cannot sustain the given workload but we cannot detect it due to $q^{a}$ value, then  the latency metrics (both event and system time latency) should increase throughout the experiment. 
% However, as we can see from our evaluations, this is not the case for our setups.
% It is also essential for the driver to distinguish unsustainable throughput and backpressure. 
% As we discussed in the paragraph above, the driver can successfully handle this issue. 
% If the queue size increases beyond $q^{a}$ but stays less than $q^{b}$, the driver starts to inspect the queue for the next $\frac{q^{b} - q^{a}}{2}  $ tuples. 
% If the queue size keeps increasing, for every such tuple, then we conclude that this is not a backpressure. 
% In fact in experiments, we show that our driver can successfully figure out the distinction between backpressure and unsustainable throughput.


% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.4\textwidth]{eps/queue}
% 	\caption{Basic intuition behind the \textit{backpressure-compatible queue}}
% 	\label{fig_queue}
% \end{figure}





\section{Workload Design}
The workload for our benchmark is derived from an online video game application at Rovio\footnote{Creator of the Angry Birds game: \url{http://www.rovio.com/}.}. Rovio continuously monitors the user actions of a given a game to ensure that their services work as expected. 
For instance, they continuously monitor the number of active users and generate alerts when this number has large drops.
Moreover, once a game has an update or receives a new feature, Rovio monitors incoming events to check whether the newly added feature is working without issues.
Rovio also tracks the in-app purchases per game, and distribution channel (e.g., Apple's AppStore, Google Play), and per in-app purchased item (e.g., a gem pack) and proposes gem packs to users as their game progresses.


\para{Dataset.}
We focus on the advertisements of gem packs. As seen in Listing 1, we have two data streams $i)$~the \texttt{purchases} stream, which contains tuples of purchased gem packs along with the purchase time, the user that made the purchase and the gem pack that was bought and $ii)$~the \texttt{ads} stream which contains a stream of proposals of gem packs to users, at given time instants. We used synthetic data, which we generate with our data generator.

\para{Queries.}
The first query that we use is an aggregation query. More specifically, we need to have a sliding window of revenue made from each gem pack. The template we use to generate such queries can be found in Listing 1.

The second query that we use is a typical use-case of correlating advertisements with their revenue. As we can see in the bottom of Listing 1, each user is presented with a specified proposal to buy a gem pack at a given time instant. We join this stream with the stream of purchases in order to find which of the proposed gems has been bought, as a result of proposing the gem to users. 



% To evaluate performance of SDPSs based on industrial setup, we need to take into account real-life scenarios in our benchmarking framework. 
% Besides evaluating the given queries, we benchmark different windowing semantics of SDPSs being global and partitioned windows. 
% Moreover, we conduct experiments when the SDPS gets more throughput than it can sustain, which is another possible scenario in industrial setup. 
% Furthermore, we analyze the systems under test with  different window sizes. 
% In addition, we simulate peaks and skewed input data which are yet another possible scenarios in online video games. 
% We present more scenarios in Appendix section. 

\begin{figure}
\begin{lstlisting}[
language=SQL,
showspaces=false,
basicstyle=\small,
commentstyle=\color{gray}
label=list2,
caption={Query templates used by our workloads.},
captionpos=b]

# Streams
PURCHASES(userID, gemPackID, price, time)
ADS(userID, gemPackID, time)

# Windowed Aggregation Query
SELECT SUM(price)
FROM   PURCHASES [Range r, Slide s] 
GROUP  BY gemPackID

# Windowed Join Query
SELECT p.userID, p.gemPackID, p.price
FROM   PURCHASES [Range r, Slide s] as p, 
       ADS       [Range r, Slide s] as a, 
WHERE  p.userID = a.userID AND
       p.gemPackID = a.gemPackID
\end{lstlisting}
\end{figure}

==> Stream Benchmarks ICDE18/6_Evaluation.tex <==
%!TEX root = icde2018.tex
\section{Evaluation}
\label{eval}
In this section, we evaluate the performance of three streaming systems, namely Storm 1.0.2, Spark 2.0.1, and Flink 1.1.3.
Due to the large number of parameters and variables, it is not possible not include all the experimental results in this paper. 
Instead, we present the most interesting results.

\subsection{System setup}
% Throughout the paper, we use cluster size only for SUT nodes, excluding the driver nodes. 
% If one experiment runs shorter than another, it means the former experiment has higher throughput than the latter. 
% We present  throughput of SUT as the number of successfully ingested tuples per second. 
% The data generation speed of each DI is equal to $\frac{sustainable\ throughput \ of \  SDPS}{number \ of \ DIs}$. 
% For example, if SUT performs with 400K/s and driver has 16 DIs, this means that the system ingests 400K tuples per second  from 16 parallel DIs each of which generates data with 25K/s. 
% Data generation speed is same for all DIs. 
% The driver determines  the data generation rate of all DIs according to SUT's sustainability and  determines the number of DIs by increasing  them until the SUT's performance doesn't improve. 
Our cluster consists of 20 nodes, each equipped with 2.40GHz Intel(R) Xeon(R) CPU  E5620  with 16 cores and 16GB RAM. The network bandwidth is 1Gb/s. We use a dedicated master for the streaming systems and an equal number of workers and driver nodes (2, 4, and 8). 
All nodes' system clocks in the cluster are synchronized via a local NTP server. Each data generator generates 100M events with constant speed using 16 parallel instances.
We generate events with normal distribution on key field.


% We utilize processing time windows in the experiments as the results were very similar to the experiments with event time windows.
% We select $q^{a}$ to be 5\% and $q^{b}$ 10 \% of the overall input. 
% Although we conducted experiments with lower values of the particular variables, it was hard to detect the systems' MST. 
% The reason is that  the systems under test use pull-based mechanism to get data from DQS, so  the smaller the queue size the more difficult to test SUT's upper limit workload. 
% Especially, detecting the difference between backpressure and  unsustainable workload with lower $q^{a}$ values is challenging. 



We use 25\% of the input data as a warmup. 
% So, in all experiments we exclude the first 25\% of output. 
We enable  backpressure  in all systems, that is, we do not allow the systems to ingest more input than they can process and crash during the experiment. 
If the SUT drops one or more connections to the data generator queue, then the driver halts the experiment with the conclusion that the SUT cannot sustain the given throughput. 
Similarly, in real-life if the system cannot sustain the user feed and drops connection,  this is considered as a failure. 



% We adopt queries from Listing 1 as representative queries for stream processing especially in online gaming scenarios. 
% We also conduct experiments for queries in Listing 2 in appendix. 
% The real-time sliding windowed aggregation and windowed join queries are the ones that distinguish SDPS from batch processing system. 
% Moreover, the use-cases are taken from real scenarios. 
Throughout the experiments, if the behavior of the system is similar with different parameters, we select the most interesting figures or features due to the limited space. 






\para{Tuning the systems.} \label{sec:tuning}
Tuning the engines' configuration parameters is important to get a good performance for every system.
% There are several properties for each SDPS, that need to be tuned to customize the given use-case. 
We adjust the buffer size  to ensure a good balance between throughput and latency.
% For example, in Flink the buffer size has to be adjusted properly to ensure a good balance between throughput and latency. 
Although selecting low buffer size can result in a low processing-time latency, the event-time latency of tuples may increase as they will be queued in the driver queues instead of the buffers inside the streaming system. 
Moreover, we adjust the block interval for partitioning the RDDs in Spark.  
% In Spark the block interval for partitioning the RDDs is one key aspect to tune the system for the given use-case. 
The number of RDD partitions a single mini-batch  is bounded by $\frac{batch \ Interval}{block \ Interval}$. 
As the cluster size increases, decreasing the block interval can increase the parallelism. 
One of the main reasons that Spark scales up very well is the partitioning of RDDs. 
However, depending on the use-case, the optimal number of RDD partitions can change. 
In Storm the number of workers, executors, and buffer size are the  configurations (among many other) that need to be tuned to get the best performance. 
% Similar to Flink, choosing the buffer size is a key to balance between latency and throughput. 
For all systems,  choosing the right level or parallelism is essential to balance between good resource utilization and network or resource exhaustion.

% We want to stress that the MST is not the same as an engine's highest throughput. 
% As stated above, we are interested in measuring maximum sustainable  throughputs of SUTs in this paper. 
% We adjusted Spark's block interval to achieve a better parallelism on RDD level and the highest sustainable throughput. 
Storm introduced the  backpressure feature in recent releases; however, it is not mature yet. 
With high workloads, it is possible that the backpressure stalls the topology, causing spouts to stop emitting tuples. 
Moreover, we notice that Storm  drops some connections to the data queue when tested with high workloads with backpressure disabled, which is not acceptable according to the real world use-cases. 
Dropping connections due to high throughput is considered  a system failure.





\subsection{Performance Evaluation}
% \textbf{Experiment 1: Windowed operations.}
% When talking about the windowed queries, we should take the system architecture into the consideration. 
% For example, Spark gathers the data in window and then parallelizes the computation within a single window. 
% Basically, it enables querying a single large window. 
% We call it a $global$  $window$. 
% Storm and Flink on the other hand, first partitions the data and then creates windows. 
% As a result, the window size is strictly equal or smaller than the size of a global window. 
% The equality condition appears  when input data is skewed with only single key. 
% We call this type $partitioned$ $window$. 
% There is no coordination between parallel partitioned windows. 
% Moreover, there is no ordering guarantee on processing the parallel partitioned windows.
% Spark supports only global windows but Flink and Storm support both global and partitioned windows. 


    \begin{table}
    \centering
        \begin{tabular}{llllll}\toprule
            &\textbf{2-node}  & \textbf{4-node} & \textbf{8-node}\\\midrule
            Storm & 0.4 M/s & 0.69 M/s & 0.99 M/s \\
            Spark & 0.38 M/s & 0.64 M/s & 0.91 M/s \\
            Flink & 1.2 M/s & 1.2 M/s & 1.2 M/s\\
        \end{tabular}
        \caption{Sustainable throughput for windowed aggregations}
        \vspace{-2em}
        \label{tab_th_agg}
    \end{table} 
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    \begin{table*}
	\resizebox{\textwidth}{!} {\begin{tabular}{ c |c c c c | c c c c | c c c c}\toprule
			& & & \textbf{2-node}  & & & & \textbf{4-node} & & & & \textbf{8-node}\\
			& \textit{avg} & \textit{min} & \textit{max} & \textit{quantiles (90,95,99)} & \textit{avg} & \textit{min} & \textit{max} & \textit{quantiles (90,95,99)} & \textit{avg} & \textit{min} & \textit{max} & \textit{quantiles (90,95,99)} \\\midrule
			Storm & 1.4 &0.07 &  5.7 & (2.3, 2.7, 3.4) & 2.1 & 0.1 & 12.2 & (3.7, 5.8, 7.7) & 2.2 & 0.2 & 17.7 & (3.8, 6.4, 9.2) \\
			Storm(90\%) & 1.1 & 0.08 & 5.7 & (1.8, 2.1, 2.8) & 1.6 & 0.04 & 9.2 & (2.9, 4.1, 6.3) & 1.9 & 0.2 & 11 & (3.3, 5, 7.6)\\
			Spark & 3.6 & 2.5 & 8.5 & (4.6, 4.9, 5.9) & 3.3 & 1.9 & 6.9 & (4.1, 4.3, 4.9) & 3.1 & 1.2 & 6.9 & (3.8, 4.1, 4.7)\\
			Spark(90\%) & 3.4 & 2.3 & 8 & (3.9, 4.5, 5.4) & 2.8 & 1.6 & 6.9 & (3.4, 3.7, 4.8) & 2.7 & 1.7 & 5.9 & (3.6, 3.9, 4.8)\\
			Flink & 0.5 & 0.004 & 12.3 & (1.4, 2.2, 5.2) & 0.2 & 0.004 & 5.1 & (0.6, 1.2, 2.4) & 0.2 & 0.004 & 5.4 & (0.6, 1.2, 3.9)\\
			Flink(90\%) & 0.3 & 0.003 & 5.8 & (0.7, 1.1, 2) & 0.2 & 0.004 & 5.1 & (0.6, 1.3, 2.4)  & 0.2 & 0.002 & 5.4 & (0.5, 0.8, 3.4)\\
	\end{tabular}}
	\caption{Latency statistics, avg, min, max, and quantiles (90, 95, 99) in seconds for windowed aggregations}
	\vspace{-2em}
	\label{tab_lat_agg}
\end{table*} 

















\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_2node_th_max_ts}

        \caption{Storm, 2-node,  max   throughput }
    \end{subfigure}\hspace{-2mm}%
    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_4node_th_max_ts}

        \caption{Storm, 4-node,  max   throughput }
    \end{subfigure}\hspace{-2mm}%
    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_8node_th_max_ts}

        \caption{Storm, 8-node,  max   throughput }
                 \label{fig_storm_agg_8node_th_max_ts}
    \end{subfigure}



    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_2node_th_max_ts}

        \caption{Spark, 2-node,  max   throughput }
    \end{subfigure}\hspace{-2mm}%
    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_4node_th_max_ts}

        \caption{Spark, 4-node,  max   throughput }
    \end{subfigure}\hspace{-2mm}%
    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_8node_th_max_ts}

        \caption{Spark, 8-node,  max   throughput }
         \label{fig_spark_agg_8node_th_max_ts}
    \end{subfigure}



    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_2node_th_max_ts}

        \caption{Flink, 2-node,  max   throughput }
                \label{flink_agg_2node_th_max_ts}

    \end{subfigure}\hspace{-2mm}%
    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_4node_th_max_ts}

        \caption{Flink, 4-node,  max   throughput }
    \end{subfigure}\hspace{-2mm}%
    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_8node_th_max_ts}

        \caption{Flink, 8-node,  max   throughput }
        
    \end{subfigure}




    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_2node_th_90_ts}

        \caption{Storm, 2-node,   90\%- throughput }
    \end{subfigure}\hspace{-2mm}%
    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_4node_th_90_ts}

        \caption{Storm, 4-node,  90\%- throughput }
                        \label{fig_storm_agg_8node_th_max_ts}
    \end{subfigure}\hspace{-2mm}%
    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_8node_th_90_ts}

        \caption{Storm, 8-node,  90\%- throughput }
                \label{fig_storm_agg_8node_th_90_ts}
    \end{subfigure}



    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_2node_th_90_ts}

        \caption{Spark, 2-node,   90\%- throughput }
    \end{subfigure}\hspace{-2mm}%
    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_4node_th_90_ts}

        \caption{Spark, 4-node,   90\%- throughput }
    \end{subfigure}\hspace{-2mm}%
    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_8node_th_90_ts}

        \caption{Spark, 8-node,   90\%- throughput }
        
    \end{subfigure}



    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_2node_th_90_ts}

        \caption{Flink, 2-node,   90\%- throughput }
        \label{fig_flink_agg_2node_th_90_ts}
    \end{subfigure}\hspace{-2mm}%
    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_4node_th_90_ts}

        \caption{Flink, 4-node,   90\%- throughput }
    \end{subfigure}\hspace{-2mm}%
    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_8node_th_90_ts}

        \caption{Flink, 8-node,  90\% throughput }
        
    \end{subfigure}

        \caption{Windowed aggregation latency distributions in time series}
        \vspace{-1em}
                \label{fig_ts_agg}
\end{figure*}










\para{Experiment 1: Windowed Aggregations.}
% We benchmark  partitioned windowed aggregations with Storm and Flink and compare it with Spark's global windowed aggregations. 
We use an  aggregation query (8s, 4s), 8 seconds window length and 4 seconds window slide, for our first evaluations.
 Table \ref{tab_th_agg} shows the sustainable throughput of the SDPSs. 
We use a four second batch-size for  Spark, as it can sustain the  maximum throughput with this configuration. 
We identify that Flink's performance is bounded by network bandwidth with    4- or more node cluster configuration. 
Storm's and Spark's performance in terms of throughput are comparable, with Storm outperforming Spark by approximately 8\% in all configurations.
% but the 14-node one, in which all systems' throughput is bounded by the network bandwidth.





    %  \setlength{\tabcolsep}{0.1em} % for the horizontal padding
% \begin{table*}
% 	\resizebox{\textwidth}{!} {\begin{tabular}{ c |c c c c | c c c c | c c c c | c c c c }\toprule
% 			& & & \textbf{2-node}  & & & & \textbf{4-node} & & & & \textbf{8-node} & & & & \textbf{14-node} \\
% 			& \textit{avg} & \textit{min} & \textit{max} & \textit{quantiles (90,95,99)} & \textit{avg} & \textit{min} & \textit{max} & \textit{quantiles (90,95,99)} & \textit{avg} & \textit{min} & \textit{max} & \textit{quantiles (90,95,99)}  & \textit{avg} & \textit{min} & \textit{max} & \textit{quantiles (90,95,99)} \\\midrule
% 			Storm & 1.4 &0.07 &  5.7 & (2.3, 2.7, 3.4) & 2.1 & 0.1 & 12.2 & (3.7, 5.8, 7.7) & 2.2 & 0.2 & 17.7 & (3.8, 6.4, 9.2)  & 2.9 & 0.2 & 19.1 & (3.8, 8.4, 13.2) \\
% 			Storm(90\%) & 1.1 & 0.08 & 5.7 & (1.8, 2.1, 2.8) & 1.6 & 0.04 & 9.2 & (2.9, 4.1, 6.3) & 1.9 & 0.2 & 11 & (3.3, 5, 7.6) & 2.6 & 0.2 & 13.7 & (3.8, 6.4, 9.2) \\
% 			Spark & 3.6 & 2.5 & 8.5 & (4.6, 4.9, 5.9) & 3.3 & 1.9 & 6.9 & (4.1, 4.3, 4.9) & 3.1 & 1.2 & 6.9 & (3.8, 4.1, 4.7) & 3.6 & 1.2 & 7.1 & (4.2, 4.3, 5.5)\\
% 			Spark(90\%) & 3.4 & 2.3 & 8 & (3.9, 4.5, 5.4) & 2.8 & 1.6 & 6.9 & (3.4, 3.7, 4.8) & 2.7 & 1.7 & 5.9 & (3.6, 3.9, 4.8) & 2.6 & 1.7 & 6.1 & (3.8, 4, 4.5)\\
% 			Flink & 0.5 & 0.004 & 12.3 & (1.4, 2.2, 5.2) & 0.2 & 0.004 & 5.1 & (0.6, 1.2, 2.4) & 0.2 & 0.004 & 5.4 & (0.6, 1.2, 3.9) & 0.3 & 0.002 & 6 & (0.6, 1.7, 4.5)\\
% 			Flink(90\%) & 0.3 & 0.003 & 5.8 & (0.7, 1.1, 2) & 0.2 & 0.004 & 5.1 & (0.6, 1.3, 2.4)  & 0.2 & 0.002 & 5.4 & (0.5, 0.8, 3.4) & 0.3 & 0.002 & 6 & (0.5, 0.7, 4.4)\\
% 	\end{tabular}}
% 	\caption{Latency statistics, avg, min, max, and quantiles (90, 95, 99) in seconds for windowed aggregations}
% 	\vspace{-2em}
% 	\label{tab_lat_agg}
% \end{table*} 



% \setlength{\tabcolsep}{0.9em} % for the horizontal padding


Table \ref{tab_lat_agg} shows the latency measurements of windowed aggregations. 
We conduct experiments with maximum and 90\%-workloads. 
% and report $avg$, $min$, $max$, and  quantiles (90,95,99) over the results. 
The latencies shown in this table correspond to    the workloads given in Table \ref{tab_th_agg}. 
In most cases, where the network bandwidth is not a bottleneck, we can see a significant decrease in latency when lowering the throughput by 10\%. 
This shows that the sustainable throughput saturates the system.
% For example, Flink's metrics shown in Table  \ref{tab_lat_agg} change more than the metrics of other systems when lowering the throughput. 
% The reason is that it pulls the data from DQS more periodically than other systems so that the queue size does not get beyond the limits. 
% Below, we conduct another set of experiments about pull graphs of systems from data sources.




% Flink has the best $min$ and $avg$ latencies. 
% Although its $max$ latency is way above its $min$, from quantile values we can conclude that those values can be considered as outliers. 
% The main reason for having such a high $max$ latency is associated with the buffer size. 
% The large buffer size enables high throughput; on the other hand, it can cause some tuples to have high latencies. 
% For example, with a larger buffer size the tuple resides in buffer longer until the buffer gets filled and flushes. 
% With 4- and more node cluster configurations, we can see that there is a slight difference in Flink's latency statistics between  the maximum and 90\%-throughputs. 
% The reason is that this workload is not the MST but is bounded by the network bandwidth. 


As we see from Table \ref{tab_lat_agg},  Spark has a higher latency than Storm and Flink but it exhibits less variation in $avg$, $min$, and $max$ latency measurements. 
Because Spark processes tuples in mini-batches, the tuples within the same batch have similar latencies and, therefore, there is little difference among the measurements. 
Moreover, transferring data from Spark's block manager to DStream by creating RDDs adds additional overhead that results in higher $avg$ latencies for Spark compared to Flink and Storm. 

The $avg$ and $max$ latencies increase in Storm with increasing workload and cluster size, while in Spark we see the opposite behavior, which means Spark can partition the data (RDDs) better in a bigger distributed environments. 
However, from the quantile values we can conclude that the $max$ latencies of Storm  can be considered as outliers.

Figure \ref{fig_ts_agg} shows the windowed aggregation latency distributions over time.
In all cases, we can see that the fluctuations are lowered when decreasing the throughput by 10\%. 
While in Storm and in Flink it is hard to detect the lower bounds of latency as they are close to zero, in Spark the upper and lower boundaries are more stable and clearly noticeable. 
The reason is that a Spark job's characteristics are  highly dependent on the batch size and this determines the clear upper and lower boundaries for the latency. 
The smaller the batch size, the lower the latency and throughput. 
To have a stable and efficient configuration in Spark, the mini-batch processing time should be less than the batch interval. 
We determine the most fluctuating system to be Flink in  2-node setup and Storm in 8-node setup  as shown in Figures \ref{flink_agg_2node_th_max_ts} and \ref{fig_storm_agg_8node_th_max_ts}. 
Those fluctuations show the behaviour of backpressure. 
% For the same experiment with 90\% of the maximum throughput, we notice that the fluctuations are significantly reduced as shown in  Figures \ref{fig_flink_agg_2node_th_90_ts} and \ref{fig_storm_agg_8node_th_90_ts}.
% As we discussed above, 4- and more node experiments in Flink are network bound; therefore, these experiments do not fully utilize the Flink nodes and thus have a lower variance in latency. 


Spark has a mini-batch based architecture and splits the input query into multiple sub-queries, which get executed in separate jobs. 
%So, the number of batch jobs for each batch-time interval   is at least one. 
To analyze this from the logical query plan perspective,  each RDD has a $transformation()$ method. 
Each $transformation()$ method produces one or more RDDs of any type that can be expressed in Scala. 
Moreover, each $transformation()$ may contain several $sub$-$transformations$. 
As a result, coordination and pipelining mini-batch jobs and their stages creates extra overhead for Spark as the relationship between consequent RDDs in a job pipeline is not necessarily one-to-one. 
For example,  we use $reduceByKey()$ to parallelize the stages of the mini-batch within a  window. 
It is transformed into two subsequent RDDs: first a ShuffledRDD and then a MapPartitionsRDD. 
In Flink and Storm, on the other hand, this is just single step both in  logical and  physical query plan. 




% \textbf{Global Windowed Aggregations.}
% As we mentioned above, in global windowed aggregations a SDPS collects the data and parallelizes a query for  data inside window. 
% As a result, the system should be able to manage and parallelize large size windows. 
% Because Spark only supports global windowed aggregations, we enable the global window aggregation semantics in Flink and Storm and compare with Spark. 
% In Flink and Storm, for all types of global windowed queries, the performance of the system is bounded by the performance of a single slot of a machine, meaning it does not scale. 
% The reason lies under the design option of a system. 
% That is, supporting  querying big windows and coordinating the sub-queries of a given query is costly. 
% For Query 1 (8s, 4s) with global windowed aggregation, we measured the throughput 480K/s for Flink and 200K/s for Storm. 
% As we mentioned above, these measurements does not improve when SUT scales. 
% From Table \ref{tab_th_agg}, we can see that with a 2-node cluster configuration Flink's  global windowed aggregation performs better than  Spark and Storm. 
% However, Spark improves the performance as it scales.

% Spark performs worse with less  computing units because it adopts blocking operators. 
% As the system scales out, this limitation becomes no longer a dominating factor. 
% Flink having record at a time architecture, avoids blocking operators. 
% For example, the $reduce$ operation  is a non-blocking operator in Flink. 
% As a result, the system sacrifices some use-cases which need blocking $reduce$, to achieve  a better performance. 
% Internally, Storm also has a similar architecture; however, the semantics of an operator is highly dependent on its implementation. 
% For example, one implementation of window reduce operator can output the results  continuously, while another can chose to perform so in bulk. 
% In Query 2, the   $reduce$ and $join$ operators in Spark, on the other hand,  have to wait until the result of the parent operator is available and system has constructed a new RDD. 















































    \begin{table}
    \centering
        \begin{tabular}{lllll}\toprule
            &\textbf{2-node}  & \textbf{4-node} & \textbf{8-node}\\\midrule
            Spark & 0.36 M/s & 0.63 M/s & 0.94 M/s  \\
            Flink & 0.85 M/s & 1.12 M/s & 1.19 M/s  \\
        \end{tabular}
        \caption{Sustainable throughput  for windowed joins. }
        \vspace{-2em}
                 \label{tab_th_join}
    \end{table} 
























\begin{figure*}
	
	\centering
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{eps/spark_join_2node_th_max_ts}
		
		\caption{Spark, 2-node, max  throughput}
		\label{fig_spark_join_2node_th_max_ts}
	\end{subfigure}%
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{eps/spark_join_4node_th_max_ts}
		
		\caption{Spark, 4-node, max  throughput }
		\label{fig_spark_join_4node_th_max_ts}
	\end{subfigure}%
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{eps/spark_join_8node_th_max_ts}
		
		\caption{Spark, 8-node, max  throughput }
		\label{fig_spark_join_8node_th_max_ts}
	\end{subfigure}
	
	
	
	
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{eps/flink_join_2node_th_max_ts}
		
		\caption{Flink, 2-node, max  throughput}
		\label{flink_join_2node_th_max_ts}
	\end{subfigure}%
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{eps/flink_join_4node_th_max_ts}
		
		\caption{Flink, 4-node, max  throughput }
		\label{flink_join_4node_th_max_ts}
	\end{subfigure}%
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{eps/flink_join_8node_th_max_ts}
		
		\caption{Flink, 8-node, max  throughput }
		\label{flink_join_8node_th_max_ts}
	\end{subfigure}
	
	
	
	
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{eps/spark_join_2node_th_90_ts}
		
		\caption{Spark, 2-node,  90\%-throughput}
	\end{subfigure}%
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{eps/spark_join_4node_th_90_ts}
		
		\caption{Spark, 4-node,  90\%-throughput }
	\end{subfigure}%
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{eps/spark_join_8node_th_90_ts}
		
		\caption{Spark, 8-node,  90\%-throughput }
	\end{subfigure}
	
	
	
	
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{eps/flink_join_2node_th_90_ts}
		
		\caption{Flink, 2-node,  90\%-throughput}
		\label{flink_join_2node_th_90_ts}
	\end{subfigure}%
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{eps/flink_join_4node_th_90_ts}
		
		\caption{Flink, 4-node,  90\%-throughput }
	\end{subfigure}%
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{eps/flink_join_8node_th_90_ts}
		
		\caption{Flink, 8-node,  90\%-throughput }
	\end{subfigure}
	
	\caption{Windowed join latency distributions in time series}
	\label{fig_ts_join}
\end{figure*}






























    % \setlength{\tabcolsep}{0.1em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.0}% for the vertical padding
	\begin{table*}
		\resizebox{\textwidth}{!} {\begin{tabular}{ l|c c c c | c c c c | c c c c}\toprule
				& & & \textbf{2-node}  & & & & \textbf{4-node} & & & & \textbf{8-node} \\
				& \textit{avg} & \textit{min} & \textit{max} & \textit{quantiles (90,95,99)} & \textit{avg} & \textit{min} & \textit{max} & \textit{quantiles (90,95,99)} & \textit{avg} & \textit{min} & \textit{max} & \textit{quantiles (90,95,99)}\\\midrule
				Spark & 7.7 & 1.3 & 21.6 & (11.2, 12.4, 14.7) & 6.7 & 2.1 & 23.6 & (10.2, 11.7, 15.4) & 6.2 & 1.8 & 19.9 & (9.4, 10.4, 13.2)\\
				Spark(90\%) & 7.1 & 2.1 & 17.9 & (10.3, 11.1, 12.7) & 5.8 & 1.8 & 13.9 & (8.7, 9.5, 10.7) & 5.7 & 1.7 & 14.1 & (8.6, 9.4, 10.6)\\
				Flink & 4.3 & 0.01 & 18.2 & (7.6, 8.5, 10.5) & 3.6 & 0.02 & 13.8 & (6.7, 7.5, 8.6) & 3.2 & 0.02 & 14.9 & (6.2, 7, 8.4)\\
				Flink(90\%) & 3.8 & 0.02 & 13 & (6.7, 7.5, 8.7) & 3.2 & 0.02 & 12.7 & (6.1, 6.9, 8)  & 3.2 & 0.02 & 14.9 & (6.2, 6.9, 8.3)\\
		\end{tabular}}
		\caption{Latency statistics, avg, min, max and quantiles (90, 95, 99) in seconds for windowed joins}
		\vspace{-1em}
		\label{tab_lat_join}
	\end{table*} 
	
% 	\setlength{\tabcolsep}{0.9em} % for the horizontal padding






\para{Experiment 2: Windowed Joins.}
We use the windowed join query from Listing 1  to benchmark Spark and Flink.
Storm provides a windowing capability but there is no built-in windowed join operator. 
Initially, we tried Storm's Trident v2.0  abstrac\-tion, which has built-in windowed join features. 
However, Trident computed incorrect results as we increased the batch size. 
Moreover, there is a lack of support for Trident in the Storm community. 
As an alternative, we implemented a simple version of a windowed join in Storm. 
Comparing it with Spark and Flink, which have advanced memory and state management features, leads to unfair comparisons. 
We implemented a na\"ive join in Storm and examined the sustainable throughput to be 0.14 million events per second and measured an average latency of 2.3 seconds  on a 2-node cluster. 
However, we faced memory issues and topology stalls on larger clusters. 
As a result, we focus on Flink and Spark for the windowed join benchmarks.

% Throughout the experiments, we found important points that need to be taken into consideration while performing windowed joins over streams. 
First, depending on the selectivity of the input streams to the join operator, vast amount of results can be produced. Sink operators can be a bottleneck in this case. 
% We are assuming that the result sink is a file system. 
Second, the vast amount of results of a join operator can cause the network to be a bottleneck. 
% This can happen if we output the results to shared file system. 
% If the result size is large, then the network becomes a bottleneck. 
To address this issue, we decreased the selectivity of the input streams. 
In general, the experimental results for windowed joins are similar to the experiments with windowed aggregations. 

Table \ref{tab_th_join} shows the  sustainable throughput of the systems under test. 
Flink's throughput for an 8-node cluster configuration is bounded by network bandwidth. 
The network saturation limit was 1.2 million events per second in windowed aggregations. 
The reason for the difference is that there is more network traffic as the result size is larger in windowed joins than in windowed aggregations. 
Tab\-le \ref{tab_lat_join} shows the latency statistics for windowed joins. 
We can see that  
in all cases Flink outperforms Spark in all parameters. 
To ensure the stability of the system, the runtime of each mini-batch should be less than batch size in Spark. 
Otherwise, the queued mini-batch jobs will increase over time and the system will not be able to sustain the throughput. 
However, we see from Table \ref{tab_th_join} that the latency values for Spark are higher than mini-batch duration (4 sec). 
The reason is that we are measuring the event-time latency. So, the additional latency is due to tuples' waiting in the queue.
% We can observe that systems under test saturate the network on 14-node cluster with Query 1 and on 13-node cluster with Query 2. 
% The reason is that the output of join queries is significantly more than aggregation queries.
























































Figure \ref{fig_ts_join} shows the windowed join latency distributions as time-series. 
In contrast to windowed aggregations, we experienced substantial fluctuations in Spark.
Also we experienced a significant latency increase in Flink when compared to windowed aggregation experiments.
The reason is that windowed joins are   more expensive than windowed aggregations. 
However, the spikes are significantly reduced with 90\% workload. 


Similar to  windowed aggregations, in  windowed joins Spark's major disadvantage is having blocking operators. 
Another limitation is coordination and scheduling overhead across different RDDs. 
For example, for  windowed joins Spark  produces CoGroupedRDD, MappedValuesRDD, and FlatMappedValuesRDD in different stages of the job. 
Each of these RDDs have to wait for the parent RDDs to be complete before their initialization. 
Flink on the other hand, performs operator chaining in  query optimization part to avoid  unnecessary data migration. 

















% \textbf{Experiment 3: Unsustainable throughput.}
% Providing the MST to SDPSs is essential as otherwise the performance of the systems can degrade. 
% We experienced on average 5-10 \% performance decrease on 20\% more throughput than a system can sustain. 
% We conducted experiments with Query 1 and  Query 2. 
% In general the decrease in overall throughput is dominated by the time interval where the system is unstable, meaning the system cannot find the best input data rate. 
% This is directly related with backpressure implementation of particular systems. 
% For example, when we executed Query 1  on 2 nodes with 20\% over-saturated workload, the overall throughput of the Storm, Spark, and Flink decreased by 6\%, 5\%, 3\%  respectively. 
% With the same parameters on Query 2, we examined approximately 1.5 times more performance decrease. 
% We experienced that with over-saturated workloads,  as the window size gets large and window slide and buffer size gets smaller, Storm's probability to drop the sockets increases. 









\para{Experiment 3: Queries with large window.}
Window size and window slide have a significant impact on the SUT's performance. 
% Here we talk about partitioned windowed operations as Spark is single winner in global windows in scale. 
One interesting observation is that with  increasing window size Spark's throughput decreases significantly given the same batch size. 
For example, for the aggregation query, with window length and slide 60 seconds, Spark's throughput decreases by 2 times and $avg$ latency increases by 10 times given a 4-seconds batch size. 
However, with higher batch sizes, Spark can handle  higher workloads and big windows sacrificing low latencies. 
We find that the main reason for Spark's decreasing performance is caching. 
We cache the windowed operation results to be usable in later stages of a job. 
However, especially with windowed join queries, the cache operation consumes the memory aggressively. 
Internally when a task gets a record for processing, it checks if the record is marked for caching. 
If yes, all the following records of the particular RDD will be sent to memory store of block manager. 
Spark will spill the memory store to disk once it is full. 
As a result, we disabled the caching. 
However, then we experienced the performance decreased due to the repeated  computation. 
Finally, after implementing Inverse Reduce Function, to account for old data going out of window, we managed to overcome this performance issues. 



Storm, on the other hand, can handle the large window  operations if the user has advanced data structures that can spill to disk when needed. 
Otherwise, we encountered memory exceptions. 
Flink (as well as Spark) has built-in data structures that can spill to disk when needed. 
However, this does not apply for the operations inside the UDFs, as Flink treats UDFs as blackbox. 
Analyzing the implementation of windowed aggregates in Flink we conclude that it cannot share aggregate results among different sliding windows. 
As Flink computes aggregates on-the-fly and not after window closes, this limitation is not a dominating factor in overall performance. 













\para{Experiment 4: Data skew.}
Data skew is yet another concern to be addressed  by SDPSs.
% When choosing the right SDPS for online gaming scenarios, data skew  should also be taken into consideration, as  in production environment  data distribution can be unpredictable. 
We analyzed the systems under test with extreme skew, namely their ability to handle data of a single key. 
In Flink and Storm, the performance of the system is bounded by the performance of a single slot of a machine, meaning it does not scale. The reason lies under the design option of a system. For aggregation query, we measured the throughput 0.48 M/s for Flink and 0.2 M/s for Storm. As we mentioned above, these measurements does not improve when SUT scales.


Spark, on the other hand, can handle skewed data efficiently. We experienced 0.53 M/s sustainable throughput for Spark in a 4-node cluster. 
Spark outperforms both engines  for the  aggregation query  in a 4- or more node cluster. 
For the join query, on the other hand, both Spark and Flink cannot  handle skewed data well. 
That is, Flink often becomes unresponsive in this test. 
Spark, on the other hand, exhibits very high latencies. 
The main reason is that the memory is consumed quite fast and backpressure mechanism lacks to perform efficiently. 
% To emphasize this, we show a small portion the the latency time series graph of our experiments. 
% As can be seen from Figure \ref{ev_sys_skew}, Spark continuously ingests the input data to system despite high system time latency. 
In these experiments, we decreased the join operator's selectivity to make sure that data transfer and I/O are not a bottleneck. 


One reason for performance difference between Spark and Flink with skewed data  lies on how the systems compute aggregations. 
Flink and Storm use one slot per operator instance. So, if the input data is skewed, this architecture can cause performance issues. 
Spark  has a slightly different architecture.
In Spark, forcing all partitions  to send their reduced value to a specific computing slot can easily cause a network to become a bottleneck when partition size is big. Therefore, Spark adopts tree reduce and tree aggregate communication pattern to minimize the communication and data shuffling. This is the main reason that makes Spark perform better with skewed input data.

\begin{figure*}
	\centering
	
	\begin{subfigure}[b]{0.19\textwidth}
		\includegraphics[width=\textwidth]{eps/storm_peak_agg_1}
		
		
		\caption{Storm aggregation }
	\end{subfigure}\hspace{-1mm}%
	\begin{subfigure}[b]{0.19\textwidth}
		\includegraphics[width=\textwidth]{eps/spark_peak_agg_1}
		
		
		\caption{ Spark aggregation} 
	\end{subfigure}\hspace{-1mm}%
	\begin{subfigure}[b]{0.19\textwidth}
		\includegraphics[width=\textwidth]{eps/flink_peak_agg_1}
		
		
		\caption{ Flink aggregation}
	\end{subfigure}\hspace{-1mm}%
	\begin{subfigure}[b]{0.19\textwidth}
		
		\includegraphics[width=\textwidth]{eps/spark_peak_join_1}

		\caption{Spark join}
		\label{peaks_spark_join}
	\end{subfigure}\hspace{-1mm}%
	\begin{subfigure}[b]{0.19\textwidth}
		
		\includegraphics[width=\textwidth]{eps/flink_peak_join_1}
		
		\caption{ Flink join} 
	\end{subfigure}
	\caption{Event-time latency on workloads with fluctuating data arrival rate.}
	\label{peaks}
\end{figure*}






\begin{figure}
	\centering
	
	\begin{subfigure}[b]{0.24\textwidth}
		\includegraphics[width=\textwidth]{eps/storm_system_more_th_1}
		
		\caption{Event time}
	\end{subfigure}\hspace{-1mm}%
	\begin{subfigure}[b]{0.24\textwidth}
		\includegraphics[width=\textwidth]{eps/storm_system_more_th_2}
		
		\caption{Processing time}
	\end{subfigure}
	
	\caption{Comparison between event  and processing-time  latency of Spark with unsustainable throughput}

	\label{more_th}
\end{figure}











\begin{figure*}
	\centering
	
	\begin{subfigure}[b]{0.28\textwidth}
		\includegraphics[width=\textwidth]{eps/storm_agg_2node_th_max2_ts}
		\includegraphics[width=\textwidth]{eps/storm_2node-system_2}
		
		\caption{Storm} 
	\end{subfigure}\hspace{-1mm}%
	\begin{subfigure}[b]{0.28\textwidth}
		\includegraphics[width=\textwidth]{eps/spark_agg_2node_th_max_2_ts}
		\includegraphics[width=\textwidth]{eps/spark_system_latency_2}
		
		\caption{Spark} 
	\end{subfigure}\hspace{-1mm}%
	\begin{subfigure}[b]{0.28\textwidth}
		\includegraphics[width=\textwidth]{eps/flink_agg_2node_th_max_2_ts}
		\includegraphics[width=\textwidth]{eps/flink_system_latency_1}
		
		\caption{Flink}
	\end{subfigure}\hspace{-1mm}%
	\caption{Comparison between event (top row) and processing-time (bottom row) latency}
	\label{event_vs_system_latency}
\end{figure*}



















\begin{figure*}
	\centering
	
	\begin{subfigure}[b]{0.3\textwidth}
		\includegraphics[width=\textwidth]{eps/storm_pull_pg}
		
		
		\caption{Storm} 
	\end{subfigure}%
	\begin{subfigure}[b]{0.3\textwidth}
		\includegraphics[width=\textwidth]{eps/spark_pull_pg}
		
		
		\caption{Spark} 
	\end{subfigure}%
	\begin{subfigure}[b]{0.3\textwidth}
		\includegraphics[width=\textwidth]{eps/flink_pull_pg}
		
		
		\caption{ Flink} 
	\end{subfigure}
	
	\caption{Throughput graphs of systems under test}
	\label{pull_graph}
\end{figure*}


Spark performs worse with less computing units (3- or less node) than Flink or Storm because it has blocking operators. As the system scales out, this limitation becomes no longer a dominating factor. Flink avoids blocking operators. For example, the reduce operation is a non-blocking operator in Flink. As a result, the system sacrifices some use-cases which need blocking reduce, to achieve a better performance. Internally, Storm also has a similar architecture; however, the semantics of an operator is highly dependent on its implementation. For example, one implementation of window reduce operator can output the results continuously, while another can chose to perform so in bulk. 
% In Query 2, the reduce and join operators in Spark, on the other hand, have to wait until the result of the parent operator is available and system has constructed a new RDD.























\begin{figure*}
	\centering
	
	\begin{subfigure}[b]{0.35\textwidth}
		\includegraphics[width=\textwidth]{eps/storm_bytes_in}
		\includegraphics[width=\textwidth]{eps/storm_load_one}
		\caption{Storm }
	\end{subfigure}%
	\begin{subfigure}[b]{0.27\textwidth}
		\includegraphics[width=\textwidth]{eps/spark_bytes_in}
		\includegraphics[width=\textwidth]{eps/spark_load_one}
		\caption{Spark }
	\end{subfigure}%
	\begin{subfigure}[b]{0.27\textwidth}
		\includegraphics[width=\textwidth]{eps/flink_bytes_in}
		\includegraphics[width=\textwidth]{eps/flink_load_one}
		\caption{Flink }
	\end{subfigure}
	
	\caption{Network (top row) CPU  (bottom row) usages  of systems in a 4-node cluster.}
	\vspace{-2em}
	\label{fig_cpu_network_metrics}
\end{figure*}









\begin{figure}
	\centering
		\begin{subfigure}[b]{0.34\textwidth}
				\includegraphics[width=\textwidth]{eps/scheduler1}

		\caption{Throughput}
	\end{subfigure}
	\begin{subfigure}[b]{0.34\textwidth}
				\includegraphics[width=\textwidth]{eps/scheduler2}

		
		\caption{Scheduler delay} 
	\end{subfigure}\hspace{-1mm}%
	
	\caption{Scheduler delay (top row) vs. throughput (bottom row) in Spark.}
	\label{scheduler}
\end{figure}














\para{Experiment 5: Fluctuating workloads.}
We analyze the systems under test with fluctuating workloads. 
We simulate spikes for all systems both for aggregation and join queries. 
We start the benchmark with a workload of 0.84 M/s  then decrease it to 0.28 M/s and increase again after a while. 
As we can see from Figure \ref{peaks}, Storm is  most susceptible system for fluctuating workloads. 
Spark and Flink have competitive behavior with windowed aggregations. 
However, for windowed joins, Flink can handle spikes better. 
One reason behind this behavior is the difference between the systems' backpressure mechanism. 
As we mentioned above, Spark can be thought as a chain of jobs with multiple stages. 
Starting from the final RDD, each stage checks its backwards to ensure lazy evaluation. 
As a result, once the stage is overloaded passing this information to upstream stages works in the order of job stage execution time; however, this time is in the order of tuples in Flink. 
We conduct experiments with different cluster and buffer sizes as well. As we increase the buffer or cluster size  the spikes  get smoother; however, the overall $avg$ latency increases. 







































\para{Experiment 6: Event-time vs processing-time latency.}
\label{event_vs_system}
% In this paper, we introduce a new definition of latency for SDPSs. 
% It is required to conduct a  comparative analysis of event time, system time and system-provided latencies. 
% System time latency is the time interval between a tuple's ingestion at a SUT and its emission from the sink operator of the SUT, with our  technique to evaluate latencies of stateful operators. 
% System-provided latency is the metric we obtain from SDPS. 
% The latency metrics inside the systems provide end-to-end $avg$ latency. 
% One issue is that we cannot see the tuple based latency when using system metrics. 
% Another issue is that the calculation of system-provided metrics might not be the same among different systems. 
% So, it would be biased to utilize this metric when benchmarking different systems. 
% Another issue is that, especially for windowed operations system-provided latency metrics  gives higher latencies than actual  system latency. 
% The reason is that, the system cannot track which input tuples contribute to a given output tuple, so it computes average of both input and output tuple timestamps. 
% Event time latency, on the other hand, is the end-to-end latency between a tuple's event time and its emission time from the sink operator of SUT, with our latency evaluation technique of stateful operators. 
Figure \ref{event_vs_system_latency} shows the comparison between the processing-time and event-time latency. 
We conduct  experiments with aggregation query (8s,4s) on a 2-node cluster. 
Even with a small cluster size,  we can see from Figure \ref{event_vs_system_latency} that there is a significant difference between event and  processing-time  latencies. 
% To be more specific, Storm has 1034, 1201, 1407 ms, Spark has 1040, 2491, 3394 ms, and  Flink has 254, 351, 563 ms system time, system-provided, and event time latencies respectively. 
As a result, we can see that with Spark, input tuples spend most of the time in driver queues. 
% Because Storm Spout is pure pull based, the tuples spend significant amount of time inside the system, inside operator buffers. 
% Flink has a difference between event and system time latency in orders of magnitude. 
% The reason is that backpressure affects only event time latency. 
% We examined the similar behavior with large cluster sizes and with windowed join queries as well.
We didn't examine any significant changes in results with different cluster configurations and with join query.

To emphasize the necessity of our definition of latency, we draw reader's attention to Figure \ref{more_th}, which shows  event time and processing-time latencies for Spark when the system is extremely overloaded. 
This is not a specific behavior for Spark but we observed similar graphs for all systems. 
As we can see from the figures, the processing-time latency is significantly lower than event-time latency. 
The reason is that when the SUT gets overloaded, it starts backpressure and lowers the data ingestion rate to stabilize  the end-to-end system latency. 
We can see that the SUT accomplished this goal as the latency stays stable. 
However, the event-time latency keeps increasing as the input tuples wait  in the queues. 
This is just one scenario where we can draw \textit{unrealistic} or \textit{incorrect} conclusions when using traditional processing-time latency for streaming systems. 







% \begin{figure}
% 	\centering
	
% 	\begin{subfigure}[b]{0.24\textwidth}
% 		\includegraphics[width=\textwidth]{eps/spark_skewed_join_1}
		
% 		\caption{Event time}
% 	\end{subfigure}\hspace{-1mm}%
% 	\begin{subfigure}[b]{0.24\textwidth}
% 		\includegraphics[width=\textwidth]{eps/spark_skewed_join_2}
		
% 		\caption{System time}
% 	\end{subfigure}
	
% 	\caption{Comparison between event and system time latency of Spark with skewed input data}

% 	\label{ev_sys_skew}
% \end{figure}

\para{Experiment 7: Observing backpressure.}
Backpressure is shown in Figures  \ref{fig_spark_join_2node_th_max_ts}, \ref{fig_spark_join_4node_th_max_ts}, \ref{fig_spark_join_8node_th_max_ts}, 	\ref{flink_join_2node_th_max_ts}, \ref{flink_join_4node_th_max_ts}, \ref{flink_join_8node_th_max_ts}, and \ref{flink_agg_2node_th_max_ts}. 
Moreover, our driver can also observe short-term spikes (Figures \ref{fig_storm_agg_8node_th_max_ts}, \ref{peaks_spark_join}) and  continuous fluctuations (Figure \ref{flink_join_2node_th_90_ts}). 
Furthermore, we can observe a wide range of sustainable $avg$ latencies from 0.2 to 6.2 seconds and from 0.003 seconds $min$ latency to 19.9 seconds $max$ latency.


% \textbf{Fault tolerance.}
% Measuring the SDPSs' fault tolerance is  well explored problem \cite{lopez2016performance}. 
% Because measuring throughput and latency is orthogonal to performing fault tolerance measurements, we  refer to the benchmark results to previous results. 
% In short, Spark is more robust to node failures than the other systems.












\para{Experiment 8: Throughput graphs.}
While analyzing the  performance of systems it is essential to inspect their throughput over time. 
As we separate the throughput calculation clearly from the SUT, we retrieve this metric from the driver. 
Figure \ref{pull_graph} shows the sustainable throughput graphs for the aggregation query (8s, 4s). 
We examined  similar behavior in other window settings and for the  join query as long as the workload is maximum sustainable. 
As we can see, Spark and Storm pulls data from the source in a more fluctuating way  than Flink. 
Despite having a high data pull rate or throughput, Flink has less fluctuations. 
When we lower the workload, both Flink and Spark have stable data pull rates; however, Storm still exhibits significant fluctuations. 

The reason for highly fluctuating throughput for Storm is that it lacks an efficient backpressure mechanism to find a near-constant data ingestion rate. 
% So,  the system cannot adjust the stable buffer fill/purge rate for all receivers. 
The main reason for fluctuation in Spark is the deployment of several jobs at the same batch interval. 
Spark has an $action()$ method on each RDD; the number of jobs at any time will be equal to the number of $action()$ method calls. 
Each job retrieves the data into its input buffers and fires. 
Until a job is finished, its input rate is limited. 
It is the DagScheduler's job to coordinate and schedule all running jobs. 
As a result, we can see a highly fluctuating throughput for Spark. 
Flink, on the other hand, benefits from its internally incremental computation mechanism (like Spark), tuple at a time semantics and efficient backpressure mechanism.






































\para{Resource usage statistics.} Figure \ref{fig_cpu_network_metrics} shows the resource usages of the SUTs. 
The below graphs in  Figure \ref{fig_cpu_network_metrics} show the CPU load during the experiment. 
% The CPU load is the number of kernel level threads  that are runnable and queued while waiting for CPU resources, averaged over one minute. 
The above graphs in Figure \ref{fig_cpu_network_metrics}  show the network usage of the SUTs. 
Because the overall result is similar, we show the systems' resource utilization graphs  for the aggregation query  in a 4-node cluster. 
Because Flink's performance is bounded by the network, we can see that CPU load is least. 
Storm and Spark, on the other hand, use approximately 50\% more CPU clock cycles than Flink. As we can see from Figure \ref{scheduler}, the scheduler overhead is one bottleneck for Spark's performance. 
Initially, Spark ingests more tuples  than it can sustain. 
Because of the scheduler delay, backpressure fires and limits the input rate. 
Whenever there is even a short spike in the input rate, we can observe a similar behavior in the scheduler delay.

%This results in having competitively higher throughout than Spark. 
% We perform experiments with different parallelism settings, block, buffer, and batch sizes, as we explained in Tuning the Systems subsection. 
% For example, increasing block and buffer size improves the throughput but results in long-lasting jobs. 
% Especially for join queries this can result in long job queues. 
% Increasing parallelism improves the throughput  but this is highly dependent on the query. 
% Throughout our experiments, we tune the systems to find the best combination of parameters for each system.
% One reason behind Spark's efficient CPU usage is its automation, transparent resource usages, and many internal optimizations   \cite{sparkcodegen}. 
% For example, Spark handles incremental state management, optimizations with code generation, and dynamic memory management efficiently and transparent to user. 


% \textbf{More scenarios.}
% We conducted experiments in a more complex scenarios with Query 3 from Listing 2. 
% The main purpose is to inspect the engines' query optimization with non-trivial queries and their scaling capabilities.
% One key finding is that  both Flink and Spark supports  operator chaining both In the logical and the physical query graph. 
% For example, Flink  chains operators  (e.g., two subsequent map transformations) if the operation is possible. 
% However, optimizations like join ordering, automatic intermediate result materialization (or caching), subgraph sharing, fission and etc. 
% are not available in neither systems. 

% Another key finding is that with a more complex query the performance of the systems stay  at the same proportion as the fundamental queries like windowed aggregation and windowed joins. 
% We conducted experiments up to 20-node cluster configuration with Query 3 for all systems. 
% We observed that with increasing number of computing nodes Spark outperforms Storm. 
% For example, with 20 nodes Spark achieved a 1.5 higher throughput than Storm. 
% Due to space restrictions, we do not provide detailed numbers here. 




% Moreover, we tested the systems with lower workloads than they can sustain. 
% For all  systems the $avg$ latency increases with the smaller workloads given the same buffer size and batch interval. 
% We had to tune the buffer size and batch interval for each workload to lower the latency. 
% However, in real industrial scenario this is not the case. 
% So, once the workload decreases the system should not be stopped and tuned for a particular workload but it should perform so automatically. 



% \begin{lstlisting}[
% language=SQL,
% showspaces=false,
% basicstyle=\scriptsize,
% numbers=left,
% numberstyle=\tiny,
% commentstyle=\color{gray}
% label=list3,
% caption={More complex query},
% captionpos=b]
% GET INPUT  l (window length) 
% and s (window slide)
% S_1 = UNION  {s_1, s_2, ..., s_m}
% S_2 = UNION {s_m, s_m+1, ..., s_n}
% S_3 = UNION  {s_1, s_2, ..., s_n}
% Query_3 = 
% 1.UPDATE S_1, S2: enrich with a new field = 
% cnt,  the country name of geo location
% 2.T=SELECT AVG(R.price)
% FROM  
% (SELECT MAX(S_2.price, S_3.price)
% FROM S_2, S_3 on window(l, s), 
% WHERE S_2.cnt = S3.cnt and S_2.ts = S3.ts)  
% as R on window(l, s)  
% GROUPBY R.geo
% WHERE R.price > 100
% 3.Execute Query 1 with input streams=T
% \end{lstlisting}




\subsection{Discussion}
% In this section we discuss our key finding from $i)$ developer, who contributes to source code, has hands-on experience with SDPSs in production environment, $ii)$ user, who owns a system or company having stream processing use-case and willing to choose better system for production and $iii)$ researcher, who conducts research on stream data processing.

% \textbf{For developers.}
% Throughout the experiments, we notice that Storm has a comparable performance  to Spark with lower numbers of nodes. 
% Storm could provide more high level abstractions  with transparent on/off-heap memory management in the engine. 
% We can see from the resource utilization graphs that the usage of low level APIs results in high CPU and network usage in the system. 
% Although Trident is a high level abstraction on top of Storm, its efficiency is much lower than Storm and with large batch sizes and it produces wrong results. 
% Moreover, Storm's backpressure mechanism needs further enhancements as it can stall the topology at high throughputs.

% Although Spark performs worse than Storm in terms of throughput, with large number of computing nodes, it outperforms Storm. 
% Its high level APIs and the dynamic memory management is better than Storm and competitive with Flink. 
% One downside of Spark is that it schedules one job at a time. 
% So there is only one active job at a time. 
% Although there is an experimental feature to start multiple mini-batch jobs at a time, this can lead to unexpected sharing of resources. 
% Moreover, Spark's backpressure mechanism was significantly improved  in recent releases but there is still need for further improvement. 

% Spark is the only system of the three tested to support caching. 
% This is an important feature especially with streaming and continuous queries. 
% If the system could automatically select a part of the DAG to cache, this would increase the system performance for non-expert users.


% Flink performs best in throughput and in $avg$ latency. 
% Flink could add a dynamic buffer management feature to change the size of buffers at runtime to reduce the latency. 
% We noticed the performance of Flink's backpressure to be the best because of its robustness and its low overhead.

% \textbf{For users.}
% There is no single winner according to the experimental results. 
% Storm's and Spark's throughputs for partitioned windowed aggregations are comparable but in terms of $avg$ latency Storm is better. 
% So if a user needs to use lower level APIs to implement custom business logic, then Storm is the best engine for windowed aggregation. 
% However, Spark reduces latency when scaling out. 
% So, when working with very large clusters Spark can outperform Storm. 
% If the data is skewed, Spark is the best system to use in scale. 
% Moreover, if the business logic needs to guarantee the order of windowed operation outputs with respect to inputs by processing global large windows, again Spark is the best choice. 
% Spark is a single winner for global windows and Flink performs better in large partitioned windows if the input data is not skewed. 


% Flink on the other hand, provides the highest throughput and the lowest  $avg$ latency with its transparent and high level APIs when working with normally distributed data w.r.t. 
% key field. 
% However, its  high $max$ latency is a limitation when compared to other systems. 
% Flink can handle peaks better than the other systems. 
% So if a user expects to have peak hours in production environment, Flink is the best choice. 
% With respect to window size Spark and Flink have competitive performance. 


% \textbf{For researchers.}
% For researchers each system provides a set of features to conduct their studies. 
% Storm provides low level APIs. 
% Researchers can use this to easily create proof of concept in their studies. 
% Novel incremental algorithms can be easily implemented without touching the system internals. 
% Moreover, new, memory friendly data structures and indexes are also best fit to be implemented in Storm. 
% Spark is the best system  for researchers working on adaptive processing. 
% The deployment of a job is not $hard$ and as persistent as in Flink or Storm. 
% It is a sequence of mini-batch jobs, so with an optimizer on top, one can perform adaptive data processing and load balancing with skewed data  efficiently with changing the DAG of the following jobs. 
% Spark is also the best system to adopt for researchers working on incremental batch and streaming  as it is the only engine among the three to allow batch and streaming queries in a single API. 
% It is internally a batch processing engine, but it successfully performs stream processing. 
% Flink is pure streaming engine. 
% Researchers working on stream data processing performance, including incremental stream computations should use Flink in their work. 




    % \begin{table}
    %     \begin{tabular}{llllll}\toprule
    %          &\textbf{Storm}  & \textbf{Spark} & \textbf{Flink} \\\midrule
    %         Data skew & $\largewhitestar$ & $\largewhitestar \largewhitestar \largewhitestar$ & $\largewhitestar \largewhitestar$   \\
    %         Fluctuating aggregation & $\largewhitestar$ & $\largewhitestar \largewhitestar \largewhitestar$ & $\largewhitestar \largewhitestar \largewhitestar$  \\
    %         Fluctuating join  & \tiny{N/A}  & $\largewhitestar \largewhitestar$ & $\largewhitestar \largewhitestar \largewhitestar$  \\
    %         Average latency & $\largewhitestar \largewhitestar$ & $\largewhitestar \largewhitestar$ & $\largewhitestar \largewhitestar \largewhitestar$  \\
    %         Bounded latency & $\largewhitestar$ & $\largewhitestar \largewhitestar \largewhitestar$ & $\largewhitestar \largewhitestar$  \\
    %         Large windows & $\largewhitestar \largewhitestar$ & $\largewhitestar  \largewhitestar$ & $\largewhitestar \largewhitestar \largewhitestar$  \\
    %         Throughput & $\largewhitestar \largewhitestar$ & $\largewhitestar \largewhitestar$ & $\largewhitestar \largewhitestar \largewhitestar$ \\
    %     \end{tabular}
    %     \caption{Summary of experiments with ratings for each system.}
    %     \vspace{-2em}
    %   \label{ratings}
    % \end{table} 






If a stream contains skewed data, then Spark is the best choice (Experiment 4).  Both Flink and Spark are very robust to fluctuations in the data arrival rate in aggregation workloads (Experiment 5).  For fluctuations in the data arrival rate on join queries, on the other hand, Flink behaves better (Experiment 5). In general, if the average latency is a priority, then Flink is the best choice (Experiments 1 and 2). On the other hand, even with higher average latency, Spark manages to bound latency better than others (Experiments 1 and 2). If a use-case contains large windows, Flink can have higher throughput with a low latency (Experiment 3). Overall, we observe that Flink has a better overall throughput both for aggregation and join queries. 
We give a definition of event and processing time latency and show the significant difference them  (Experiment 6). 






\subsection{Future work}

We plan to extend our framework along the lines of TPC database benchmarks. The main intuition is  to define both a workload of queries that should be concurrently executed  and then base the benchmark on a small number of operators that are part of that workload. In addition, we are developing a generic interface that users can plug into any stream data processing system, such as Apache Samza, Heron, and Apache Apex,  in order to facilitate and simplify benchmark SDPSs. Moreover, in depth analysis of trading SUT's increased functionality, like exactly once processing or out-of-order and late arriving data management, over better throughput/latency is another open challenge to explore.  
















==> Stream Benchmarks ICDE18/7_Conclusion.tex <==
%!TEX root = icde2018.tex
\section{Conclusions}
\label{conc}

Responding to an increasing need for real-time data processing in industry, we build a novel framework for benchmarking streaming engines with online video game scenarios. 
We identify current challenges in this area and build our benchmark to evaluate them. 
First, we give the  definition of latency of a stateful operator and a methodology to measure it. 
The solution is lightweight and does not require the use of additional systems. 
Second, we completely separate the systems under test from the driver. 
Third, we introduce a simple and novel technique to conduct  experiments with the highest sustainable workloads.
We conduct extensive experiments with the three major distributed, open source stream processing engines - Apache Storm, Apache Spark, and Apache Flink. 
In the experiments, we can see that each system has specific advantages and challenges. 
We provide a set of rules in our discussion part that can be used as a guideline to determine the requirements for a use-case.


==> Stream Benchmarks ICDE18/8_Acknowledgments.tex <==
%!TEX root = icde2018.tex
\section*{Acknowledgments}
%The authors would like to acknowledge the invaluable help of Rovio Entertainment in providing the use-cases. 
This work has been supported by the European Commission through Proteus (ref. 687691) and Streamline (ref. 688191) and by the German Ministry for Education and Research as Berlin Big Data Center BBDC (funding mark 01IS14013A). 

==> Stream Benchmarks ICDE18/Makefile <==
pdf:
	mkdir -p build
	@TEXINPUTS=.//: pdflatex -synctex=1 -interaction=nonstopmode -output-directory=build --shell-escape icde2018
all:
	mkdir -p build
	@TEXINPUTS=.//: pdflatex -synctex=1 -interaction=nonstopmode -output-directory=build --shell-escape icde2018
	bibtex build/icde2018
	pdflatex -synctex=1 -interaction=nonstopmode -output-directory=build icde2018
	pdflatex -synctex=1 -interaction=nonstopmode -output-directory=build icde2018
fig:
	rm figures/cache/*
	pdflatex -interaction=nonstopmode -output-directory build --shell-escape icde2018
clean:
	rm -rf build
	find . -type f \( -name  '*.thm' -or -name 'icde2018.pdf' -or -name '*.aux' -or -name  '*.auxlock' -or -name '*.figlist' -or -name '*eps-converted-to.pdf' -or -name '*.bbl' -or -name '*.fdb_latexmk' -or -name '*.synctex.gz' -or -name '*.blg' -or -name '*.log' -or -name '*.out' -or -name '*.toc' -or -name '*.lot' -or -name '*.lof' -or -name '*.loa' -or -name '*.fls' \) -exec rm -f '{}' \;
edit:
	subl paper.sublime-project


==> Stream Benchmarks ICDE18/temp/tex/boxplot_aggregation.tex <==
\usepgfplotslibrary{statistics}
\pgfplotsset{compat=1.8}
\usetikzlibrary{pgfplots.statistics}
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{1.2}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother


\makeatletter
\newenvironment{customlegend}[1][]{%
    \begingroup
    % inits/clears the lists (which might be populated from previous
    % axes):
    \pgfplots@init@cleared@structures
    \pgfplotsset{#1}%
}{%
    % draws the legend:
    \pgfplots@createlegend
    \endgroup
}%

% makes \addlegendimage available (typically only available within an
% axis environment):
\def\addlegendimage{\pgfplots@addlegendimage}
\makeatother



\begin{figure}

\begin{tikzpicture}

\begin{axis}[
scaled y ticks = false,
legend entries={simulation,
                measurement,
                sample 1}, 
                legend style={at={(axis cs:6.0,0.84)},anchor=south west},
boxplot/draw direction=y,
ylabel={Latency (millisecond)},
height=4cm,
boxplot={
    %
    % Idea: 
    %  place the 
    %  group 1 at 0.3333 and 0.6666
    %  group 2 at 1.3333 and 1.6666
    %  group 3 at 2.3333 and 2.6666
    %  ...
    % in a formular:
    draw position={1/4 + floor(\plotnumofactualtype/3) + 1/5*mod(\plotnumofactualtype,3)},
    %
    % that means the box extend must be at most 0.33333 :
    box extend=0.1,
},
% ... it also means that 1 unit in x controls the width:
x=1cm,
% ... and it means that we should describe intervals:
xtick={0,1,2,...,10},
ytick={0, 500,10000},
x tick label as interval,
xticklabels={%
    {\tiny 2-node \\ max th.},%
    {\tiny 2-node \\ 90 \% th.},%
    {\tiny 4-node \\ max th.},%
    {\tiny 4-node \\ 90 \% th.},%
    {\tiny 8-node \\ max th.},%
    {\tiny 8-node \\ 90 \% th.},%
},
    x tick label style={
        text width=4.5cm,
        align=center
    },
]
\addlegendimage{line legend,green}
\addlegendentry{ \textcolor{red}{\scriptsize{Storm}   }  }
\addlegendimage{line legend,blue}
\addlegendentry{\textcolor{blue}{\scriptsize{Spark}}}
\addlegendimage{line legend,blue}
\addlegendentry{\textcolor{black}{\scriptsize{Flink}}}
    % 2 node 100
\addplot[color=red,
    boxplot prepared={
      average=1407,
      lower whisker=66,
      upper whisker=5758,
      lower quartile=168,
      upper quartile=3477,
      median=1100
    },
    ] coordinates {};
    
\addplot[color=blue,
    boxplot prepared={
      average=3673,
      lower whisker=2537,
      upper whisker=8596,
      lower quartile=340,
      upper quartile=5990,
      median=2578
    },
    ] coordinates {};
    
    
\addplot[color=black,
    boxplot prepared={
      average=563,
      lower whisker=4,
      upper whisker=12328,
      lower quartile=15,
      upper quartile=5233,
      median=161
    },
    ] coordinates {};
    % 2 node 90
\addplot[color=red,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
    
    
\addplot[color=blue,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
\addplot[color=black,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
    
        % 4 node 100
    \addplot[color=red,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
    
    
\addplot[color=blue,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
\addplot[color=black,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
    
            % 4 node 90
    \addplot[color=red,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
    
    
\addplot[color=blue,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
\addplot[color=black,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};

            
            % 8 node 100
\addplot[color=red,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
    
    
\addplot[color=blue,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
\addplot[color=black,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};

            
            
             % 8 node 90
 \addplot[color=red,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2,
       average = 4.05
    },
    ] coordinates {};
    
    
\addplot[color=blue,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
\addplot[color=black,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};


\end{axis}

\end{tikzpicture}
\caption{dede}
\end{figure}


==> Stream Benchmarks ICDE18/temp/tex/flink_agg.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_2node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/flink_agg_2node_th_max_ts}

        \caption{2 Node latency with maximum throughput}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_4node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/flink_agg_4node_th_max_ts}

        \caption{4 Node latency with network bounded throughput }
    \end{subfigure}
   ~
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_8node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/flink_agg_8node_th_max_ts}

        \caption{8 Node latency with network bounded throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_2node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/flink_agg_2node_th_90_ts}

        \caption{2 Node latency with 90\% throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_4node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/flink_agg_4node_th_90_ts}

        \caption{2 Node latency with 90\% throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_8node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/flink_agg_8node_th_90_ts}

        \caption{2 Node latency with 90\% throughput }
    \end{subfigure}




        \caption{Latency of windowed aggregations for Flink}
\end{figure*}

==> Stream Benchmarks ICDE18/temp/tex/flink_join.tex <==
\begin{figure*}
   \centering
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/flink_join_2node_th_max_hist}
        \includegraphics[width=\textwidth]{eps/flink_join_2node_th_max_ts}

       \caption{2 Node latency with max throughput}
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/flink_join_4node_th_max_hist}
        \includegraphics[width=\textwidth]{eps/flink_join_4node_th_max_ts}

       \caption{4 Node latency with max throughput }
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/flink_join_8node_th_max_hist}
        \includegraphics[width=\textwidth]{eps/flink_join_8node_th_max_ts}

       \caption{8 Node latency with max throughput }
   \end{subfigure}




   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/flink_join_2node_th_90_hist}
        \includegraphics[width=\textwidth]{eps/flink_join_2node_th_90_ts}

       \caption{2 Node latency with 90\% throughput }
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/flink_join_4node_th_90_hist}
        \includegraphics[width=\textwidth]{eps/flink_join_4node_th_90_ts}

       \caption{4 Node latency with 90\% throughput }
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/flink_join_8node_th_90_hist}
        \includegraphics[width=\textwidth]{eps/flink_join_8node_th_90_ts}

       \caption{4 Node latency with 90\% throughput }
   \end{subfigure}



        \caption{Latency of windowed join for Flink}
\end{figure*}

==> Stream Benchmarks ICDE18/temp/tex/spark_agg.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_2node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/spark_agg_2node_th_max_ts}

        \caption{2 Node latency with max throughput}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_4node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/spark_agg_4node_th_max_ts}

        \caption{4 Node latency with max throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_8node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/spark_agg_8node_th_max_ts}

        \caption{8 Node latency with max throughput }
    \end{subfigure}




    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_2node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/spark_agg_2node_th_90_ts}

        \caption{2 Node latency with 90\% throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_4node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/spark_agg_4node_th_90_ts}

        \caption{4 Node latency with 90\% throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_8node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/spark_agg_8node_th_90_ts}

        \caption{8 Node latency with 90\% throughput }
    \end{subfigure}



        \caption{Latency of windowed aggregations for Spark}
\end{figure*}

==> Stream Benchmarks ICDE18/temp/tex/spark_join.tex <==
\begin{figure*}
    \centering
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/spark_join_2node_th_max_hist}
        \includegraphics[width=\textwidth]{eps/spark_join_2node_th_max_ts}

       \caption{2 Node latency with max throughput}
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/spark_join_4node_th_max_hist}
        \includegraphics[width=\textwidth]{eps/spark_join_4node_th_max_ts}

       \caption{4 Node latency with max throughput }
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/spark_join_8node_th_max_hist}
        \includegraphics[width=\textwidth]{eps/spark_join_8node_th_max_ts}

       \caption{8 Node latency with max throughput }
   \end{subfigure}




   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/spark_join_2node_th_90_hist}
        \includegraphics[width=\textwidth]{eps/spark_join_2node_th_90_ts}

       \caption{2 Node latency with 90\% throughput }
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/spark_join_4node_th_90_hist}
        \includegraphics[width=\textwidth]{eps/spark_join_4node_th_90_ts}

       \caption{4 Node latency with 90\% throughput }
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/spark_join_8node_th_90_hist}
        \includegraphics[width=\textwidth]{eps/spark_join_8node_th_90_ts}

       \caption{8 Node latency with 90\% throughput }
   \end{subfigure}



        \caption{Latency of windowed join for Spark}
\end{figure*}

==> Stream Benchmarks ICDE18/temp/tex/storm_agg.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_2node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/storm_agg_2node_th_max_ts}

        \caption{2 Node latency with max throughput}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_4node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/storm_agg_4node_th_max_ts}

        \caption{4 Node latency with max throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_8node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/storm_agg_8node_th_max_ts}

        \caption{8 Node latency with max throughput }
    \end{subfigure}




    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_2node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/storm_agg_2node_th_90_ts}

        \caption{2 Node latency with 90\% throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_4node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/storm_agg_4node_th_90_ts}

        \caption{4 Node latency with 90\% throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_8node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/storm_agg_8node_th_90_ts}

        \caption{4 Node latency with 90\% throughput }
    \end{subfigure}




        \caption{Latency of windowed aggregations for Storm}
\end{figure*}

==> Stream Benchmarks ICDE18/temp/tex/tables.tex <==
    \begin{table}[H]
        \begin{tabular}{lllll}\toprule
            &\textbf{2 Node}  & \textbf{4 Node} & \textbf{8 Node}\\\midrule
            Storm & 408K & 696K & 992K  \\
            Spark & 379K & 642K & 912K  \\
            Flink & 1230K & 1260K & 1260K  \\
            \\\bottomrule
        \end{tabular}
        \caption{Sustainable throughput for windowed aggregations. }
        \label{tab_th_agg}
    \end{table} 



    \begin{table*}
        \begin{tabular}{lllll}\toprule
            &\textbf{2 Node}  & \textbf{4 Node} & \textbf{8 Node}\\\midrule
            Storm & 1424, 66, 6297, (913, 1305, 1798) & 2043, 115, 12216, (1090, 1633, 2424) & 2260, 179, 21107, (1225, 1788, 2594) \\
            Storm(90\%) & 1109, 84, 5752, (701, 1006, 1394) & 1669, 43, 9773, (918, 1377, 2028) & 1914, 182, 11040, (1072, 1565, 2257) \\
            Spark & 3759, 2537, 9427, (3211, 3473, 3973) & 4138, 1987, 17898, (3136, 3400, 3903) & 3152, 1223, 6946, (2746, 3074, 3495)\\
            Spark(90\%) & 3418, 2354, 8005, (3149, 3239, 3739) & 2846, 1630, 6925, (2508, 2670, 3035) & 2798, 1702, 5961, (2307, 2665, 3172)\\
            Flink & 576, 4, 12328, (85, 158, 578) & 259, 4, 5132, (66, 101, 176) & 243, 4, 5528, (56, 85, 120) \\
            Flink(90\%) & 299, 3, 5826, (73, 119, 394) & 257, 3, 6790, (55, 90, 145)  & 215, 2, 7002, (55, 84, 114) \\
            \\\bottomrule
        \end{tabular}
        \caption{ Latency statistics, avg, min, max and quantiles (25, 50, 75) in milliseconds for windowed aggregations.}
         \label{tab_lat_agg}
    \end{table*} 


    \begin{table}[H]
        \begin{tabular}{lllll}\toprule
            &\textbf{2 Node}  & \textbf{4 Node} & \textbf{8 Node}\\\midrule
            Spark & 365K & 632K & 947K  \\
            Flink & 851K & 1128K & 1190K \\
            \\\bottomrule
        \end{tabular}
        \caption{Sustainable throughput for windowed joins}
                 \label{tab_th_join}
    \end{table} 



    \begin{table*}
        \begin{tabular}{lllll}\toprule
            &\textbf{2 Node}  & \textbf{4 Node} & \textbf{8 Node}\\\midrule
            Spark & 8417, 1376, 27130, (5926, 7892, 10217) & 7823, 2139, 31121, (4963, 6856, 9508) & 7590, 1841, 33976, (4682, 6454, 8964) \\
            Spark(90\%) & 7538, 2157, 27649, (5641, 7236, 9121) & 5825, 1861, 13956, (4205, 5546, 7227) & 6015, 1721, 19118, (4305, 5691, 7447)\\
            Flink & 4825, 17, 31271, (2783, 4451, 6430) & 4255, 19, 33328, (2094, 3642, 5613) & 3748, 22, 23628, (1711, 3208, 5150) \\
            Flink(90\%) & 3872, 19, 15143, (2245, 3599, 5305) & 3285, 16, 12702, (1646, 2992, 4690)  & 3336, 16, 17580, (1597, 3016, 4802) \\
            \\\bottomrule
        \end{tabular}
        \caption{Latency statistics, avg, min, max and quantiles (25, 50, 75) in milliseconds for windowed joins.}
                 \label{tab_lat_join}
    \end{table*} 


==> temp/tex/boxplot_aggregation.tex <==
\usepgfplotslibrary{statistics}
\pgfplotsset{compat=1.8}
\usetikzlibrary{pgfplots.statistics}
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{1.2}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother


\makeatletter
\newenvironment{customlegend}[1][]{%
    \begingroup
    % inits/clears the lists (which might be populated from previous
    % axes):
    \pgfplots@init@cleared@structures
    \pgfplotsset{#1}%
}{%
    % draws the legend:
    \pgfplots@createlegend
    \endgroup
}%

% makes \addlegendimage available (typically only available within an
% axis environment):
\def\addlegendimage{\pgfplots@addlegendimage}
\makeatother



\begin{figure}

\begin{tikzpicture}

\begin{axis}[
scaled y ticks = false,
legend entries={simulation,
                measurement,
                sample 1}, 
                legend style={at={(axis cs:6.0,0.84)},anchor=south west},
boxplot/draw direction=y,
ylabel={Latency (millisecond)},
height=4cm,
boxplot={
    %
    % Idea: 
    %  place the 
    %  group 1 at 0.3333 and 0.6666
    %  group 2 at 1.3333 and 1.6666
    %  group 3 at 2.3333 and 2.6666
    %  ...
    % in a formular:
    draw position={1/4 + floor(\plotnumofactualtype/3) + 1/5*mod(\plotnumofactualtype,3)},
    %
    % that means the box extend must be at most 0.33333 :
    box extend=0.1,
},
% ... it also means that 1 unit in x controls the width:
x=1cm,
% ... and it means that we should describe intervals:
xtick={0,1,2,...,10},
ytick={0, 500,10000},
x tick label as interval,
xticklabels={%
    {\tiny 2-node \\ max th.},%
    {\tiny 2-node \\ 90 \% th.},%
    {\tiny 4-node \\ max th.},%
    {\tiny 4-node \\ 90 \% th.},%
    {\tiny 8-node \\ max th.},%
    {\tiny 8-node \\ 90 \% th.},%
},
    x tick label style={
        text width=4.5cm,
        align=center
    },
]
\addlegendimage{line legend,green}
\addlegendentry{ \textcolor{red}{\scriptsize{Storm}   }  }
\addlegendimage{line legend,blue}
\addlegendentry{\textcolor{blue}{\scriptsize{Spark}}}
\addlegendimage{line legend,blue}
\addlegendentry{\textcolor{black}{\scriptsize{Flink}}}
    % 2 node 100
\addplot[color=red,
    boxplot prepared={
      average=1407,
      lower whisker=66,
      upper whisker=5758,
      lower quartile=168,
      upper quartile=3477,
      median=1100
    },
    ] coordinates {};
    
\addplot[color=blue,
    boxplot prepared={
      average=3673,
      lower whisker=2537,
      upper whisker=8596,
      lower quartile=340,
      upper quartile=5990,
      median=2578
    },
    ] coordinates {};
    
    
\addplot[color=black,
    boxplot prepared={
      average=563,
      lower whisker=4,
      upper whisker=12328,
      lower quartile=15,
      upper quartile=5233,
      median=161
    },
    ] coordinates {};
    % 2 node 90
\addplot[color=red,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
    
    
\addplot[color=blue,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
\addplot[color=black,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
    
        % 4 node 100
    \addplot[color=red,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
    
    
\addplot[color=blue,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
\addplot[color=black,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
    
            % 4 node 90
    \addplot[color=red,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
    
    
\addplot[color=blue,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
\addplot[color=black,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};

            
            % 8 node 100
\addplot[color=red,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
    
    
\addplot[color=blue,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
\addplot[color=black,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};

            
            
             % 8 node 90
 \addplot[color=red,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2,
       average = 4.05
    },
    ] coordinates {};
    
    
\addplot[color=blue,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};
\addplot[color=black,
    boxplot prepared={
      median=1,
      upper quartile=1.2,
      lower quartile=0.4,
      upper whisker=1.5,
      lower whisker=0.2
    },
    ] coordinates {};


\end{axis}

\end{tikzpicture}
\caption{dede}
\end{figure}


==> temp/tex/flink_agg.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_2node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/flink_agg_2node_th_max_ts}

        \caption{2 Node latency with maximum throughput}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_4node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/flink_agg_4node_th_max_ts}

        \caption{4 Node latency with network bounded throughput }
    \end{subfigure}
   ~
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_8node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/flink_agg_8node_th_max_ts}

        \caption{8 Node latency with network bounded throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_2node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/flink_agg_2node_th_90_ts}

        \caption{2 Node latency with 90\% throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_4node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/flink_agg_4node_th_90_ts}

        \caption{2 Node latency with 90\% throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/flink_agg_8node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/flink_agg_8node_th_90_ts}

        \caption{2 Node latency with 90\% throughput }
    \end{subfigure}




        \caption{Latency of windowed aggregations for Flink}
\end{figure*}

==> temp/tex/flink_join.tex <==
\begin{figure*}
   \centering
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/flink_join_2node_th_max_hist}
        \includegraphics[width=\textwidth]{eps/flink_join_2node_th_max_ts}

       \caption{2 Node latency with max throughput}
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/flink_join_4node_th_max_hist}
        \includegraphics[width=\textwidth]{eps/flink_join_4node_th_max_ts}

       \caption{4 Node latency with max throughput }
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/flink_join_8node_th_max_hist}
        \includegraphics[width=\textwidth]{eps/flink_join_8node_th_max_ts}

       \caption{8 Node latency with max throughput }
   \end{subfigure}




   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/flink_join_2node_th_90_hist}
        \includegraphics[width=\textwidth]{eps/flink_join_2node_th_90_ts}

       \caption{2 Node latency with 90\% throughput }
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/flink_join_4node_th_90_hist}
        \includegraphics[width=\textwidth]{eps/flink_join_4node_th_90_ts}

       \caption{4 Node latency with 90\% throughput }
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/flink_join_8node_th_90_hist}
        \includegraphics[width=\textwidth]{eps/flink_join_8node_th_90_ts}

       \caption{4 Node latency with 90\% throughput }
   \end{subfigure}



        \caption{Latency of windowed join for Flink}
\end{figure*}

==> temp/tex/spark_agg.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_2node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/spark_agg_2node_th_max_ts}

        \caption{2 Node latency with max throughput}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_4node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/spark_agg_4node_th_max_ts}

        \caption{4 Node latency with max throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_8node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/spark_agg_8node_th_max_ts}

        \caption{8 Node latency with max throughput }
    \end{subfigure}




    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_2node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/spark_agg_2node_th_90_ts}

        \caption{2 Node latency with 90\% throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_4node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/spark_agg_4node_th_90_ts}

        \caption{4 Node latency with 90\% throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/spark_agg_8node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/spark_agg_8node_th_90_ts}

        \caption{8 Node latency with 90\% throughput }
    \end{subfigure}



        \caption{Latency of windowed aggregations for Spark}
\end{figure*}

==> temp/tex/spark_join.tex <==
\begin{figure*}
    \centering
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/spark_join_2node_th_max_hist}
        \includegraphics[width=\textwidth]{eps/spark_join_2node_th_max_ts}

       \caption{2 Node latency with max throughput}
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/spark_join_4node_th_max_hist}
        \includegraphics[width=\textwidth]{eps/spark_join_4node_th_max_ts}

       \caption{4 Node latency with max throughput }
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/spark_join_8node_th_max_hist}
        \includegraphics[width=\textwidth]{eps/spark_join_8node_th_max_ts}

       \caption{8 Node latency with max throughput }
   \end{subfigure}




   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/spark_join_2node_th_90_hist}
        \includegraphics[width=\textwidth]{eps/spark_join_2node_th_90_ts}

       \caption{2 Node latency with 90\% throughput }
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/spark_join_4node_th_90_hist}
        \includegraphics[width=\textwidth]{eps/spark_join_4node_th_90_ts}

       \caption{4 Node latency with 90\% throughput }
   \end{subfigure}
   ~ 
   \begin{subfigure}[b]{0.3\textwidth}
       \includegraphics[width=\textwidth]{eps/spark_join_8node_th_90_hist}
        \includegraphics[width=\textwidth]{eps/spark_join_8node_th_90_ts}

       \caption{8 Node latency with 90\% throughput }
   \end{subfigure}



        \caption{Latency of windowed join for Spark}
\end{figure*}

==> temp/tex/storm_agg.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_2node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/storm_agg_2node_th_max_ts}

        \caption{2 Node latency with max throughput}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_4node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/storm_agg_4node_th_max_ts}

        \caption{4 Node latency with max throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_8node_th_max_hist}
         \includegraphics[width=\textwidth]{eps/storm_agg_8node_th_max_ts}

        \caption{8 Node latency with max throughput }
    \end{subfigure}




    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_2node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/storm_agg_2node_th_90_ts}

        \caption{2 Node latency with 90\% throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_4node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/storm_agg_4node_th_90_ts}

        \caption{4 Node latency with 90\% throughput }
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{eps/storm_agg_8node_th_90_hist}
         \includegraphics[width=\textwidth]{eps/storm_agg_8node_th_90_ts}

        \caption{4 Node latency with 90\% throughput }
    \end{subfigure}




        \caption{Latency of windowed aggregations for Storm}
\end{figure*}

==> temp/tex/tables.tex <==
    \begin{table}[H]
        \begin{tabular}{lllll}\toprule
            &\textbf{2 Node}  & \textbf{4 Node} & \textbf{8 Node}\\\midrule
            Storm & 408K & 696K & 992K  \\
            Spark & 379K & 642K & 912K  \\
            Flink & 1230K & 1260K & 1260K  \\
            \\\bottomrule
        \end{tabular}
        \caption{Sustainable throughput for windowed aggregations. }
        \label{tab_th_agg}
    \end{table} 



    \begin{table*}
        \begin{tabular}{lllll}\toprule
            &\textbf{2 Node}  & \textbf{4 Node} & \textbf{8 Node}\\\midrule
            Storm & 1424, 66, 6297, (913, 1305, 1798) & 2043, 115, 12216, (1090, 1633, 2424) & 2260, 179, 21107, (1225, 1788, 2594) \\
            Storm(90\%) & 1109, 84, 5752, (701, 1006, 1394) & 1669, 43, 9773, (918, 1377, 2028) & 1914, 182, 11040, (1072, 1565, 2257) \\
            Spark & 3759, 2537, 9427, (3211, 3473, 3973) & 4138, 1987, 17898, (3136, 3400, 3903) & 3152, 1223, 6946, (2746, 3074, 3495)\\
            Spark(90\%) & 3418, 2354, 8005, (3149, 3239, 3739) & 2846, 1630, 6925, (2508, 2670, 3035) & 2798, 1702, 5961, (2307, 2665, 3172)\\
            Flink & 576, 4, 12328, (85, 158, 578) & 259, 4, 5132, (66, 101, 176) & 243, 4, 5528, (56, 85, 120) \\
            Flink(90\%) & 299, 3, 5826, (73, 119, 394) & 257, 3, 6790, (55, 90, 145)  & 215, 2, 7002, (55, 84, 114) \\
            \\\bottomrule
        \end{tabular}
        \caption{ Latency statistics, avg, min, max and quantiles (25, 50, 75) in milliseconds for windowed aggregations.}
         \label{tab_lat_agg}
    \end{table*} 


    \begin{table}[H]
        \begin{tabular}{lllll}\toprule
            &\textbf{2 Node}  & \textbf{4 Node} & \textbf{8 Node}\\\midrule
            Spark & 365K & 632K & 947K  \\
            Flink & 851K & 1128K & 1190K \\
            \\\bottomrule
        \end{tabular}
        \caption{Sustainable throughput for windowed joins}
                 \label{tab_th_join}
    \end{table} 



    \begin{table*}
        \begin{tabular}{lllll}\toprule
            &\textbf{2 Node}  & \textbf{4 Node} & \textbf{8 Node}\\\midrule
            Spark & 8417, 1376, 27130, (5926, 7892, 10217) & 7823, 2139, 31121, (4963, 6856, 9508) & 7590, 1841, 33976, (4682, 6454, 8964) \\
            Spark(90\%) & 7538, 2157, 27649, (5641, 7236, 9121) & 5825, 1861, 13956, (4205, 5546, 7227) & 6015, 1721, 19118, (4305, 5691, 7447)\\
            Flink & 4825, 17, 31271, (2783, 4451, 6430) & 4255, 19, 33328, (2094, 3642, 5613) & 3748, 22, 23628, (1711, 3208, 5150) \\
            Flink(90\%) & 3872, 19, 15143, (2245, 3599, 5305) & 3285, 16, 12702, (1646, 2992, 4690)  & 3336, 16, 17580, (1597, 3016, 4802) \\
            \\\bottomrule
        \end{tabular}
        \caption{Latency statistics, avg, min, max and quantiles (25, 50, 75) in milliseconds for windowed joins.}
                 \label{tab_lat_join}
    \end{table*} 

